Converting Depth Images and Point Clouds for Feature-based Pose Estimation

In recent years, depth sensors have become more and more affordable and have found their way into a growing amount of robotic systems. However, mono- or multi-modal sensor registration, often a necessary step for further processing, faces many challenges on raw depth images or point clouds. This paper presents a method of converting depth data into images capable of visualizing spatial details that are basically hidden in traditional depth images. After noise removal, a neighborhood of points forms two normal vectors whose difference is encoded into this new conversion. Compared to Bearing Angle images, our method yields brighter, higher-contrast images with more visible contours and more details. We tested feature-based pose estimation of both conversions in a visual odometry task and RGB-D SLAM. For all tested features, AKAZE, ORB, SIFT, and SURF, our new Flexion images yield better results than Bearing Angle images and show great potential to bridge the gap between depth data and classical computer vision. Source code is available here: https://rlsch.github.io/depth-flexion-conversion.

==> content/eval/slam_tum_ate_1.tex <==
\renewcommand{\minval}{1.04}
\renewcommand{\midval}{65.965}
\renewcommand{\maxval}{130.89}
\begin{table}[bt]
	\centering
	\caption{\acs{ATE} [\(cm\)] of \acs{RGB-D} \acs{SLAM} on TUM~\acs{RGB-D} 1/2}
	\label{tab:ate:tum:1}
	\begin{tabular}{l|r|r|r|r}
		Variant               &      fr1/xyz &     fr1/desk &    fr1/floor &     fr1/room \\
		\hline
		\flexionnxn{3}        &    \cs{3.82} &   \cs{28.41} &   \cs{83.16} &  \cs{130.89} \\
		\flexionnxn{5}        &    \cs{3.15} &   \cs{21.25} & \csbf{64.96} &   \cs{69.27} \\
		\flexionnxn{7}        &    \cs{3.11} &   \cs{14.25} & \csbf{66.26} & \csbf{62.37} \\
		\flexionnxn{9}        &    \cs{3.15} &  \csbf{9.18} &   \cs{75.19} &  \cs{122.43} \\
		\flexionnxn{11}       &    \cs{3.16} & \csbfu{8.82} &   \cs{74.13} &  \cs{129.73} \\
		\flexionnxn{13}       &    \cs{3.11} &  \csbf{9.53} &   \cs{75.99} &  \cs{106.49} \\
		\hline
		\acs{BA} horizontal   &  \csbf{2.64} &   \cs{67.64} &   \cs{75.68} &   \cs{87.96} \\
		\acs{BA} vertical     &    \cs{2.84} &   \cs{67.78} &   \cs{74.76} & \csbf{69.06} \\
		\acs{BA} diagonal     &    \cs{3.02} &   \cs{61.91} &   \cs{86.48} &   \cs{73.59} \\
		\acs{BA} antidiagonal &  \csbf{2.73} &   \cs{54.45} &   \cs{83.55} &   \cs{70.75} \\
		\hline
		Color                 & \csbfu{1.04} &   \cs{40.68} & \csbfu{4.70} & \csbfu{7.30} \\
	\end{tabular}
\end{table}



==> content/eval/slam_tum_ate_2_cm.tex <==
\renewcommand{\minval}{12.25}
\renewcommand{\midval}{114.78}
\renewcommand{\maxval}{217.31}
\begin{table}[bt]
    \centering
    \caption{\acs{ATE} [\(cm\)] of \acs{RGB-D} \acs{SLAM} on TUM~\acs{RGB-D} 2/2}
    \label{tab:ate:tum:2}
    \setlength\tabcolsep{5pt}
    \begin{tabular}{@{\hskip 2pt}r@{\hskip 1pt}l|r|r|r|r|r|r}
        \multicolumn{2}{c|}{\multirow{4}{*}{Variant}} 	& fr2/ 	& fr3/ 		& \multicolumn{4}{c}{} \\
                                                        &       & large     & long      & \multicolumn{4}{c}{fr2/pioneer\_} \\
                                                        &       & \_with    & \_office  & \multicolumn{1}{c}{\multirow{2}{*}{360}} & \multicolumn{1}{c}{\multirow{2}{*}{slam}} & \multicolumn{1}{c}{\multirow{2}{*}{slam2}} & \multicolumn{1}{c}{\multirow{2}{*}{slam3}}  \\
                                                        &       & \_loop    & \_househ  &   &   &   &   \\
        \hline
        \parbox[t][0mm][c]{3mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\flexion}}} & 
          \(_{3\times3}\)           & \csbf{112.51} &    \cs{77.78} &   \cs{182.14} &    \cs{193.81} &    \cs{215.72} &    \cs{191.96} \\
        & \(_{5\times5}\)           & \csbf{112.74} &    \cs{64.65} &   \cs{173.42} &  \csbf{187.00} &    \cs{215.59} &    \cs{181.59} \\
        & \(_{7\times7}\)           &   \cs{138.47} &  \csbf{57.36} &   \cs{159.36} &    \cs{189.14} &    \cs{215.86} &    \cs{180.19} \\
        & \(_{9\times9}\)           &   \cs{135.98} &  \csbf{61.35} & \csbf{155.12} &    \cs{187.69} &    \cs{209.96} &  \csbf{173.70} \\
        & \(_{11\times11}\)         &   \cs{136.35} &    \cs{61.68} & \csbf{156.04} &    \cs{191.79} &    \cs{210.77} &    \cs{175.66} \\
        & \(_{13\times13}\)         &   \cs{136.45} &    \cs{67.29} &   \cs{158.24} &  \csbf{184.22} &  \csbf{207.38} &  \csbf{162.06} \\ \hline
        \parbox[t][0mm][c]{3mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\acs{BA}}}} & 
        horiz. 	                    &   \cs{113.68} &    \cs{94.87} &   \cs{191.93} &    \cs{192.27} &    \cs{217.31} &    \cs{195.90} \\
        & vert.                     &   \cs{112.87} &    \cs{80.48} &            -- &    \cs{194.37} &  \csbf{205.25} &    \cs{192.58} \\
        & diag.                     &   \cs{112.87} &   \cs{192.08} &   \cs{199.31} &    \cs{192.49} &    \cs{208.10} &    \cs{190.98} \\
        & antid.                    &   \cs{142.11} &    \cs{72.79} &   \cs{196.08} &    \cs{190.69} &    \cs{212.55} &    \cs{192.80} \\ \hline
        \multicolumn{2}{c|}{Color}	& \csbfu{18.47} & \csbfu{12.37} & \csbfu{12.25} & \csbfu{137.84} & \csbfu{156.62} & \csbfu{111.26}
    \end{tabular}
\end{table}


==> content/eval/slam_tum_ate_2_m.tex <==
\begin{table}[bt]
	\centering
	\caption{\acs{ATE} [\(m\)] of \acs{RGB-D} \acs{SLAM} on TUM~\acs{RGB-D} 2/2}
	\label{tab:ate:tum:2}
	\begin{tabular}{l|r|r|r|r|r|r}
		\multirow{4}{*}{Variant} 	& fr2/ & fr3/ & \multicolumn{4}{c}{ } \\
		& large & long & \multicolumn{4}{c}{fr2/pioneer\_} \\
		& \_with	& \_office	& \multirow{2}{*}{360} & \multirow{2}{*}{slam} & \multirow{2}{*}{slam2} & \multirow{2}{*}{slam3}  \\
		& \_loop	& \_househ	&  &  &  &   \\
		\hline
		\flexionnxn{3}      &  \textbf{1.13} &           0.78 &           1.82 &           1.94 &           2.16 &           1.92 \\
		\flexionnxn{5}      &  \textbf{1.13} &           0.65 &           1.73 &  \textbf{1.87} &           2.16 &           1.82 \\
		\flexionnxn{7}      &           1.38 &  \textbf{0.57} &           1.59 &           1.89 &           2.16 &           1.80 \\
		\flexionnxn{9}      &           1.36 &  \textbf{0.61} &  \textbf{1.55} &           1.88 &           2.10 &  \textbf{1.74} \\
		\flexionnxn{11}     &           1.36 &           0.62 &  \textbf{1.56} &           1.92 &           2.11 &           1.76 \\
		\flexionnxn{13}     &           1.36 &           0.67 &           1.58 &  \textbf{1.84} &  \textbf{2.07} &  \textbf{1.62} \\ \hline
		\acs{BA} horizontal &           1.14 &           0.95 &           1.92 &           1.92 &           2.17 &           1.96 \\
		\acs{BA} vertical   &           1.13 &           0.80 &             -- &           1.94 &  \textbf{2.05} &           1.93 \\
		\acs{BA} diagonal   &           1.13 &           1.92 &           1.99 &           1.92 &           2.08 &           1.91 \\
		\acs{BA} antidiag.  &           1.42 &           0.73 &           1.96 &           1.91 &           2.13 &           1.93 \\ \hline
		Color               & \textbfu{0.18} & \textbfu{0.12} & \textbfu{0.12} & \textbfu{1.38} & \textbfu{1.57} & \textbfu{1.11}
	\end{tabular}
\end{table}


==> content/eval/slam_tum_rpe_1.tex <==
\renewcommand{\minval}{1.45}
\renewcommand{\midval}{78.985}
\renewcommand{\maxval}{156.52}
\begin{table}[bt]
	\centering
	\caption{\acs{RPE} [\(cm\)] of \acs{RGB-D} \acs{SLAM} on TUM~\acs{RGB-D} 1/2}
	\label{tab:rpe:tum:1}
	\begin{tabular}{l|r|r|r|r|r}
		Variant               &     fr1/xyz &      fr1/desk &     fr1/floor &      fr1/room \\
		\hline
        \flexionnxn{3}        &   \cs{4.87} &    \cs{37.05} &   \cs{148.76} &   \cs{152.11} \\
        \flexionnxn{5}        &   \cs{4.00} &    \cs{28.35} &   \cs{129.13} &    \cs{98.90} \\
        \flexionnxn{7}        &   \cs{3.98} &    \cs{19.39} &   \cs{124.78} &  \csbf{85.81} \\
        \flexionnxn{9}        &   \cs{4.02} &  \csbf{13.87} &   \cs{122.34} &   \cs{149.60} \\
        \flexionnxn{11}       &   \cs{4.03} & \csbfu{12.98} & \csbf{120.53} &   \cs{156.52} \\
        \flexionnxn{13}       &   \cs{3.98} &  \csbf{14.29} &   \cs{122.23} &   \cs{120.58} \\
		\hline
		\acs{BA} horizontal   & \csbf{3.43} &    \cs{78.70} &   \cs{136.50} &   \cs{124.39} \\
		\acs{BA} vertical     &   \cs{3.67} &    \cs{78.56} &   \cs{122.76} &    \cs{93.94} \\
		\acs{BA} diagonal     &   \cs{3.77} &    \cs{72.10} &   \cs{129.49} &   \cs{101.77} \\
		\acs{BA} antidiagonal & \csbf{3.55} &    \cs{66.29} & \csbf{120.89} &  \csbf{90.50} \\
		\hline
		Color 			& \csbfu{1.45} &    \cs{48.55} &  \csbfu{6.24} & \csbfu{11.31} \\
	\end{tabular}
\end{table}


==> content/eval/slam_tum_rpe_2_cm.tex <==
\renewcommand{\minval}{17.15}
\renewcommand{\midval}{151.1}
\renewcommand{\maxval}{285.05}
\begin{table}[bt]
	\centering
	\caption{\acs{RPE} [\(cm\)] of \acs{RGB-D} \acs{SLAM} on TUM~\acs{RGB-D} 2/2}
	\label{tab:rpe:tum:2}
	\setlength\tabcolsep{5pt}
	\begin{tabular}{@{\hskip 2pt}r@{\hskip 1pt}l|r|r|r|r|r|r}
		\multicolumn{2}{c|}{\multirow{4}{*}{Variant}} 	& fr2/ 	& fr3/ 		& \multicolumn{4}{c}{} \\
														& 		& large 	& long 		& \multicolumn{4}{c}{fr2/pioneer\_} \\
														& 		& \_with	& \_office	& \multicolumn{1}{c}{\multirow{2}{*}{360}} & \multicolumn{1}{c}{\multirow{2}{*}{slam}} & \multicolumn{1}{c}{\multirow{2}{*}{slam2}} & \multicolumn{1}{c}{\multirow{2}{*}{slam3}}  \\
														& 		& \_loop	& \_househ	&  &  &  &   \\
		\hline
		\parbox[t][0mm][c]{3mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\flexion}}} & 
          \(_{3\times3}\)         	&   \cs{141.11} &    \cs{93.42} &   \cs{221.44} &    \cs{243.68} &    \cs{276.94} &   \cs{259.86} \\
		& \(_{5\times5}\)         	&   \cs{143.49} &    \cs{75.81} &   \cs{211.24} &    \cs{239.85} &    \cs{284.03} & \csbf{239.41} \\
		& \(_{7\times7}\)         	&   \cs{211.79} &  \csbf{65.91} &   \cs{195.12} &  \csbf{236.84} &    \cs{282.42} & \csbf{241.34} \\
		& \(_{9\times9}\)      	  	&   \cs{251.07} &  \csbf{70.41} & \csbf{186.37} &    \cs{242.51} &    \cs{282.05} &   \cs{246.34} \\
		& \(_{11\times11}\)       	&   \cs{254.59} &    \cs{71.86} & \csbf{187.42} &    \cs{243.04} &    \cs{285.05} &   \cs{252.73} \\
		& \(_{13\times13}\)       	&   \cs{159.37} &    \cs{74.04} &   \cs{193.47} &    \cs{243.54} &    \cs{281.85} &   \cs{265.85} \\ \hline
		\parbox[t][0mm][c]{3mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\acs{BA}}}} & 
		  horiz.					&   \cs{141.68} &   \cs{122.34} &   \cs{239.75} &    \cs{239.23} &    \cs{274.45} &   \cs{274.12} \\
		& vert. 					& \csbf{137.60} &    \cs{92.36} &        --     &    \cs{248.65} &  \csbf{269.44} &   \cs{252.70} \\
		& diag. 					& \csbf{138.87} &   \cs{188.75} &   \cs{251.55} &    \cs{239.08} &  \csbf{266.47} &   \cs{250.39} \\
		& antid.					&   \cs{168.77} &    \cs{87.81} &   \cs{246.73} &  \csbf{238.23} &    \cs{277.49} &   \cs{263.00} \\ \hline
		\multicolumn{2}{c|}{Color}	& \csbfu{28.56} & \csbfu{17.15} & \csbfu{19.86} & \csbfu{112.87} & \csbfu{213.78} & \csbfu{83.88} \\
	\end{tabular}
\end{table}

==> content/eval/slam_tum_rpe_2_m.tex <==
\begin{table}[bt]
	\centering
	\caption{\acs{RPE} [\(m\)] of \acs{RGB-D} \acs{SLAM} on TUM~\acs{RGB-D} 2/2}
	\label{tab:rpe:tum:2}
	\begin{tabular}{l|r|r|r|r|r|r}
		\multirow{4}{*}{Variant} 	& fr2/ 		& fr3/ 		& \multicolumn{4}{c}{} \\
									& large 	& long 		& \multicolumn{4}{c}{fr2/pioneer\_} \\
									& \_with	& \_office	& \multirow{2}{*}{360} 	& \multirow{2}{*}{slam} & \multirow{2}{*}{slam2} & \multirow{2}{*}{slam3}  \\
									& \_loop	& \_househ	&  						&  						& 	 					 & \\
		\hline
		\flexionnxn{3}      		&           1.41 &           0.93 &           2.21 &	           2.44 &           2.77 &           2.60 \\
		\flexionnxn{5}      		&           1.43 &           0.76 &           2.11 &	           2.40 &           2.84 &  \textbf{2.39} \\
		\flexionnxn{7}      		&           2.12 &  \textbf{0.66} &           1.95 &	  \textbf{2.37} &           2.82 &  \textbf{2.41} \\
		\flexionnxn{9}      		&           2.51 &  \textbf{0.70} &  \textbf{1.86} &	           2.43 &           2.82 &           2.46 \\
		\flexionnxn{11}     		&           2.55 &           0.72 &  \textbf{1.87} &	           2.43 &           2.85 &           2.53 \\
		\flexionnxn{13}     		&           1.59 &           0.74 &           1.93 &	           2.44 &           2.82 &           2.66 \\ \hline
		\acs{BA} horizontal 		&           1.42 &           1.22 &           2.40 &	           2.39 &           2.74 &           2.74 \\
		\acs{BA} vertical   		&  \textbf{1.38} &           0.92 &             -- &	           2.49 &  \textbf{2.69} &           2.53 \\
		\acs{BA} diagonal   		&  \textbf{1.39} &           1.89 &           2.52 & 	           2.39 &  \textbf{2.66} &           2.50 \\
		\acs{BA} antidiag.  		&           1.69 &           0.88 &           2.47 &	  \textbf{2.38} &           2.77 &           2.63 \\ \hline
		Color               		& \textbfu{0.29} & \textbfu{0.17} & \textbfu{0.20} &	 \textbfu{1.13} & \textbfu{2.14} & \textbfu{0.84}
	\end{tabular}
\end{table}


==> content/eval/slam_zhang.tex <==
\renewcommand{\minval}{5.25}
\renewcommand{\midval}{29.71}
\renewcommand{\maxval}{54.17}
\begin{table}[tb]
	\centering
	\caption{Results of \acs{RGB-D} \acs{SLAM} on synthetic scene}
	\label{tab:aterpe:zhang:slam}
	\begin{tabular}{l|r|r}
		Variant               &      ATE [m] &      RPE [m] \\ \hline
		\flexionnxn{3}        &   \cs{33.64} &   \cs{40.27} \\
		\flexionnxn{5}        &   \cs{25.53} &   \cs{31.24} \\
		\flexionnxn{7}        &   \cs{12.74} &   \cs{15.79} \\
		\flexionnxn{9}        &    \cs{7.55} &  \csbf{8.67} \\
		\flexionnxn{11}       &  \csbf{7.14} &  \csbf{8.84} \\
		\flexionnxn{13}       &  \csbf{7.16} &    \cs{8.86} \\
		\flexionang           &   \cs{39.95} &   \cs{51.00} \\
		\flexionnorm          &   \cs{19.01} &   \cs{22.26} \\ \hline
		\acs{BA} horizontal   &   \cs{41.37} &   \cs{54.17} \\
		\acs{BA} vertical     &   \cs{27.00} &   \cs{32.27} \\
		\acs{BA} diagonal     &   \cs{30.11} &   \cs{35.49} \\
		\acs{BA} antidiagonal &   \cs{31.39} &   \cs{37.01} \\ \hline
		Color                 & \csbfu{5.25} & \csbfu{6.97}
	\end{tabular}
\end{table}


==> content/eval/tum_length.tex <==
\begin{table}[bt]
    \centering
    \caption{Ground truth trajectory length [\(m\)] of TUM~\acs{RGB-D}~\cite{Sturm2012a}}
    \label{tab:tum:gtlength}
    \begin{tabular}{l|r|r|r|r|r}
        Scene  & fr1/xyz & fr1/desk & fr1/floor & \multicolumn{1}{r}{fr1/room} &  \\ \cline{1-5}
        Length & 7.112   &    9.263 &    12.569 &   \multicolumn{1}{r}{15.989} &  \\
        \multicolumn{6}{c}{\vspace{-7pt}} \\
        \multicolumn{1}{r|}{fr2/large\_}& fr3/long\_of& \multicolumn{4}{c}{fr2/pioneer\_} \\
        \multicolumn{1}{r|}{with\_loop}	& fice\_househ	& 360 & slam & slam2 & slam3  \\
        \hline
        39.111 &    21.455 & 16.118 & 40.380 & 21.735 & 18.135 \\
    \end{tabular}%
\end{table}


==> content/eval/vo_zhang_ate.tex <==
\renewcommand{\minval}{3.58}
\renewcommand{\midval}{29.625}
\renewcommand{\maxval}{55.67}
\begin{table}[tb]
	\centering
	\caption{\acs{ATE} [\(m\)] of visual odometry on synthetic scene}
	\label{tab:ate:zhang:vo}
	\begin{tabular}{l|r|r|r|r}
		Variant                &        AKAZE &          ORB &         SIFT &         SURF \\ \hline
		\flexionnxn{3}         & \csbfu{3.99} &  \csbf{5.20} &    \cs{7.65} &   \cs{32.03} \\
		\flexionnxn{5}         &    \cs{7.87} &  \csbf{5.70} &  \csbf{6.45} &   \cs{30.47} \\
		\flexionnxn{7}         &    \cs{8.70} &   \cs{13.75} &    \cs{9.22} & \csbfu{5.10} \\
		\flexionnxn{9}         &  \csbf{7.13} &    \cs{6.72} &  \csbf{7.33} &  \csbf{6.10} \\
		\flexionnxn{11}        &   \cs{14.07} &   \cs{11.41} &   \cs{44.20} &   \cs{45.33} \\
		\flexionnxn{13}        &    \cs{8.66} &   \cs{16.00} &   \cs{53.87} &   \cs{41.48} \\
		\flexionang            &   \cs{40.56} &   \cs{11.05} &   \cs{40.49} &   \cs{31.04} \\
		\flexionnorm           &   \cs{19.29} &    \cs{7.63} &              &   \cs{36.74} \\
		\hline
		\acs{BA} horizontal    &   \cs{22.53} &   \cs{13.36} &   \cs{38.87} &   \cs{44.23} \\
		\acs{BA} vertical      &   \cs{11.01} &    \cs{7.44} &   \cs{42.53} &   \cs{35.16} \\
		\acs{BA} diagonal      &   \cs{11.87} &    \cs{8.00} &   \cs{44.13} &   \cs{55.67} \\
		\acs{BA} antidiagonal  &   \cs{16.72} &   \cs{14.70} &   \cs{31.28} &   \cs{27.60} \\ \hline
		Color                  &  \csbf{6.19} & \csbfu{4.89} & \csbfu{3.58} & \csbf{12.24} \\
	\end{tabular}
\end{table}

==> content/eval/vo_zhang_rpe.tex <==
\renewcommand{\minval}{46.52}
\renewcommand{\midval}{78.34}
\renewcommand{\maxval}{110.16}
\begin{table}[tb]
	\centering
	\caption{\acs{RPE} [\(m\)] of visual odometry on synthetic scene}
	\label{tab:rpe:zhang:vo}
	\begin{tabular}{l|r|r|r|r}
		Variant & AKAZE & ORB & SIFT & SURF \\
		\hline
		\flexionnxn{3}         & \csbfu{47.22} &    \cs{55.85} &    \cs{54.74} &    \cs{87.19} \\
		\flexionnxn{5}         &  \csbf{50.45} &    \cs{58.56} & \csbfu{46.52} &    \cs{67.76} \\
		\flexionnxn{7}         &    \cs{60.51} &    \cs{57.69} &    \cs{56.19} & \csbfu{49.47} \\
		\flexionnxn{9}         &    \cs{56.08} &    \cs{54.84} &  \csbf{52.55} &  \csbf{51.91} \\
		\flexionnxn{11}        &    \cs{84.75} &    \cs{83.25} &    \cs{98.54} &    \cs{60.87} \\
		\flexionnxn{13}        &    \cs{76.05} &    \cs{87.64} &   \cs{110.16} &    \cs{61.05} \\
		\flexionang            &    \cs{91.58} &    \cs{50.47} &    \cs{68.22} &    \cs{82.45} \\
		\flexionnorm           &    \cs{69.06} &    \cs{54.65} &               &    \cs{69.46} \\
		\hline
		\acs{BA} horizontal    &    \cs{69.87} &  \csbf{49.62} &    \cs{92.06} &    \cs{69.77} \\
		\acs{BA} vertical      &    \cs{57.97} &  \csbf{50.05} &    \cs{71.96} &    \cs{80.24} \\
		\acs{BA} diagonal      &    \cs{68.97} &    \cs{55.55} &    \cs{76.97} &   \cs{104.52} \\
		\acs{BA} antidiagonal  &  \csbf{55.91} & \csbfu{48.38} &    \cs{75.10} &    \cs{79.71} \\
		\hline
		Color                  &    \cs{56.11} &    \cs{53.03} &  \csbf{51.36} &  \csbf{56.95} \\
	\end{tabular}
\end{table}


==> content/formula.tex <==
\begin{equation}
    \centering
    \label{eq:flexion:n1}
    \vec{n}_{1,i,j} = \frac{\mathbf{P}_{i,j\text{--}1} - \mathbf{P}_{i,j+1}}{ \abs{\mathbf{P}_{i,j\text{--}1} - \mathbf{P}_{i,j+1}} } \times \frac{\mathbf{P}_{i\text{--}1,j} - \mathbf{P}_{i+1,j}}{ \abs{\mathbf{P}_{i\text{--}1,j} - \mathbf{P}_{i+1,j}}}
\end{equation}%
\begin{equation}
    \centering
    \label{eq:flexion:n2}
    \vec{n}_{2,i,j} = \frac{\mathbf{P}_{i\text{--}1,j\text{--}1} - \mathbf{P}_{i+1,j+1}}{\abs{\mathbf{P}_{i\text{--}1,j\text{--}1} - \mathbf{P}_{i+1,j+1}}} \times \frac{\mathbf{P}_{i\text{--}1,j+1} - \mathbf{P}_{i+1,j\text{--}1}}{\abs{\mathbf{P}_{i\text{--}1,j+1} - \mathbf{P}_{i+1,j\text{--}1}}}
\end{equation}%
\begin{figure}[t]
    \centering
    \scalebox{1}{\input{img/flexion_perspective.tex}}
    \caption{Graphical representation of the \flexion image calculation. Horizontal, vertical (blue) and diagonal, antidiagonal (orange) neighbors of \(\mathbf{P}_{i,j}\) that form the two normal vectors defining the \flexion image. Due to the curvature of the surface, horizontal/vertical neighbors define a different normal vector (\(\vec{n}_{1,i,j}\), blue) than diagonal/antidiagonal neighbors (\(\vec{n}_{2,i,j}\), orange, dashed). Thereby, the local shape of the surface influences the angle between both normal vectors that is proportional to the \flexion \(\mathcal{F}_{i,j}\).}
    \label{fig:flexion:normals}
\end{figure}% no new paragraph
These two normals usually differ and span an angle (\cref{fig:flexion:normals}).
It is to be noted that both normals \(\vec{n}_{1,i,j}\) and \(\vec{n}_{2,i,j}\) are not unit length but each factor of their cross product is. Finally, the \flexion \(\mathcal{F}_{i,j}\) at point \(\mathbf{P}_{i,j}\) is defined as
\begin{equation}
    \centering
    \label{eq:flexion:F}
    \mathcal{F}_{i,j} = \left| (\vec{n}_{1,i,j})^\top \vec{n}_{2,i,j} \right|\text{\,,}
\end{equation}
with \(\left|\cdot\right|\) being the absolute value.
Since the length of the normals are \(\abs{\vec{n}_{1,i,j}}, \abs{\vec{n}_{2,i,j}} \in [0,1]\), the value of \(\mathcal{F}_{i,j}\) is bound to \(\mathcal{F}_{i,j} \in [0, 1]\).
This value is then linearly scaled to a grayscale value analogous to \cref{eq:color_mapping}.


==> img/bearing_angle.tex <==
% !TeX root = ../root.tex

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-0.5,xscale=0.8,line width=0.75pt]

	\coordinate (c) at (145,202);
	\coordinate (P1) at (43,16);
	\coordinate (P2) at (206,7);

	\coordinate (phiradius) at ($(c)!18mm!(P1)$);
	\coordinate (betaradius) at ($(P2)!11mm!(P1)$);
	
	\draw                        (c) -- (P1) node[pos=.5,anchor=east] {\(r_{i-1,j}\)};
	\draw [{Latex[length=3mm]}-] ($(P1)!1mm!(c)$) -- (c);
	\draw                        (c) -- (P2) node[pos=.6,anchor=west] {\(r_{i,j}\)};
	\draw [{Latex[length=3mm]}-] ($(P2)!1mm!(c)$) -- (c);
	\draw [dashed,gray]   (P1) -- (P2) ;

	\begin{scope}
		\path[clip] (c) -- (P1) -- (P2) -- cycle;
		\node () [draw,circle through=(phiradius)] at (c) {};
		\node () [draw,circle through=(betaradius),color=cb-red] at (P2) {};
	\end{scope}

	\begin{scope}[yscale=1.28,xscale=0.8]
		\fill[fill=black] (P1) circle (1.2mm);
		\fill[fill=black] (P2) circle (1.2mm);
	\end{scope}

	\node[anchor=east] at (P1) {$\mathbf{P}_{i-1,j}$};
	\node[anchor=west] at (P2) {$\mathbf{P}_{i,j}$};
	\node[anchor=north] at (c) {$\mathbf{C = (0,0,0)^\top}$};
	
	\coordinate (P1C) at ($(P1)!0.50!(c)$);
	\coordinate (beta) at ($(P2)!0.19!(P1C)$);
	\node[color=cb-red] at (beta) {\acl{bang}};

	\coordinate (P1P2) at ($(P1)!0.55!(P2)$);
	\coordinate (dphi) at ($(c)!0.23!(P1P2)$);
	\node[] at (dphi) {\acl{angres}};

\end{tikzpicture}


==> img/bearing_understand_shading.tex <==
\tikzset{every picture/.style={line width=0.75pt}}

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1,color=black]

	\coordinate (g1) at (50,100);
	\coordinate (g2) at (300,100);
	
	\coordinate (c) at (20,34);

	\begin{scope}[draw,shape=circle, xshift=20, yshift=14,color=blue]

		\tikzmath{\x1=9; \y1=20; \y2=30; \y0=100;}

		\node (v2) at (\x1+1*9:\y0+3*\y1+3*\y2) {};
		\node (v3) at (\x1+2*9:\y0+2*\y1+1*\y2) {};
		\node (v4) at (\x1+3*9:\y0+1*\y1) {};
		\node (v5) at (\x1+4*9:\y0) {};
		\draw (c) -- (v2)
	  		  (c) -- (v3)
			  (c) -- (v4)
			  (c) -- (v5);
	\end{scope}

	\coordinate (b1) at (intersection of c--v5 and g1--g2);
	\coordinate (b2) at (intersection of c--v4 and g1--g2);
	\coordinate (b3) at (intersection of c--v3 and g1--g2);
	\coordinate (b4) at (intersection of c--v2 and g1--g2);

	\begin{scope}
		\path[clip] (c) -- (b1) -- (b2) -- cycle;
		\node () [draw,circle,minimum size=8mm,color=cb-darkblue] at (b1) {};
	\end{scope}
	
	\begin{scope}
		\path[clip] (c) -- (b3) -- (b4) -- cycle;
		\node () [draw,circle,minimum size=11mm,color=cb-orange] at (b3) {};
	\end{scope}

	\fill (c) node[below,yshift=-2mm] {\(\mathbf{C}\)} circle (1mm);

	\draw (c) to (b1);
	\draw (c) -- (b2);
	\draw (c) -- (b3);
	\draw (c) -- (b4);

	\draw [line width=3] (g1) -- (g2);

	\draw (b1) node [anchor=south,xshift=0.5mm,yshift=-0.1mm][font=\scriptsize,color=cb-darkblue] {\acl{bang}};
	\draw (b3) node [anchor=south,xshift=1.0mm,yshift=0.5mm][font=\scriptsize,color=cb-orange] {\(\acl{bang}'\)};
\end{tikzpicture}

==> img/flexion_angle_decrease2.tex <==
\tikzset{every picture/.style={line width=0.75pt}}

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
	\def\cx{80}
	\def\cy{40}
	
	\coordinate (g1) at (100-2,108);
	\coordinate (g2) at (330+2,108);
	\draw [line width=2] (g1) -- (g2) ;
	
	\coordinate (c) at (\cx,\cy);
	\fill (c) node[below,yshift=-2mm] {\(\mathbf{C}\)} circle (1mm);
	
	\begin{scope}[draw,shape=circle, xshift=\cx, yshift=\cy,color=blue]
		\tikzmath{\x1=5;
			 \d1=15;
			 \y1=20; \y2=20; \y0=100;}
		
		\node (v2) at (\x1+1*\d1:\y0+3*\y1+3*\y2) {};
		\node (v3) at (\x1+2*\d1:\y0+2*\y1+1*\y2) {};
		\node (v4) at (\x1+3*\d1:\y0+1*\y1) {};
		\node (v5) at (\x1+4*\d1:\y0) {};
	\end{scope}
	
	\coordinate (b1) at (intersection of c--v5 and g1--g2);
	\coordinate (b2) at (intersection of c--v4 and g1--g2);
	\coordinate (b3) at (intersection of c--v3 and g1--g2);
	\coordinate (b4) at (intersection of c--v2 and g1--g2);
	\path (b1) +(0,100) coordinate (b1x);
	\path (b2) +(0,100) coordinate (b2x);
	\path (b3) +(0,100) coordinate (b3x);
	\path (b4) +(0,100) coordinate (b4x);

	\draw (c) to (b1);
	\draw (c) -- (b2);
	\draw (c) -- (b3);
	\draw (c) -- (b4);

\begin{scope}[yshift=80]
		
		\def\cy2{70}
		\coordinate (c) at (\cx,\cy2);
		\fill (c) node[below,yshift=-2mm] {\(\mathbf{C}\)} circle (1mm);
		
		\begin{scope}[draw,shape=circle, color=green] % shift = coordinates of C
			\tikzset{shift={(\cx,\cy2)}};
			\def\angle{10}
			\node (w1) at (-\angle:200) {};
			\node (w2) at (+\angle:200) {};
			\node (w3) at (0:200) {};
		\end{scope}
		
		
		\coordinate (s1) at (w1);
		\coordinate (s2) at (w2);
		\draw (c) -- (s1);
		\draw (c) -- (s2);
		
		\coordinate (p9)  at (intersection of c--w3 and b1--b1x);
		\coordinate (p10) at (intersection of c--w3 and b2--b2x);
		\coordinate (p11) at (intersection of c--w3 and b3--b3x);
		\coordinate (p12) at (intersection of c--w3 and b4--b4x);
		
		\begin{scope}[dashed, opacity=0.0]
			\path[clip] (c) -- (s1) -- (s2) -- cycle;
			\node (circle1) [draw,circle through=(p9)] at (c) {};
			\node (circle2) [draw,circle through=(p10)] at (c) {};
			\node (circle3) [draw,circle through=(p11)] at (c) {};
			\node (circle4) [draw,circle through=(p12)] at (c) {};
		\end{scope}
		
		\coordinate (p1) at (intersection of circle1 and c--s1);
		\coordinate (p2) at (intersection of circle2 and c--s1);
		\coordinate (p3) at (intersection of circle1 and c--s2);
		\coordinate (p4) at (intersection of circle2 and c--s2);
		
		\coordinate (p5) at (intersection of circle3 and c--s1);
		\coordinate (p6) at (intersection of circle4 and c--s1);
		\coordinate (p7) at (intersection of circle3 and c--s2);
		\coordinate (p8) at (intersection of circle4 and c--s2);
		
		\draw [opacity=0.4, dashed, color=gray, line width=0.3pt] (b1) -- ($(b1)!33mm!(p9)$);
		\draw [opacity=0.4, dashed, color=gray, line width=0.3pt] (b2) -- ($(b2)!33mm!(p10)$);
		\draw [opacity=0.4, dashed, color=gray, line width=0.3pt] (b3) -- ($(b3)!33mm!(p11)$);
		\draw [opacity=0.4, dashed, color=gray, line width=0.3pt] (b4) -- ($(b4)!33mm!(p12)$);
	
		\coordinate (i1) at (intersection of p1--p4 and p2--p3);
		\coordinate (i2) at (intersection of p5--p8 and p7--p6);
		\begin{scope}[color=cb-blue, draw opacity=1]
			
			\draw [-latex,opacity=0.8] (intersection of b2--b2x and c--w3) -- (intersection of b1--b1x and c--w3);
			\draw [-latex,opacity=0.8] (intersection of i1--i1|-b1 and c--s1) -- (intersection of i1--i1|-b1 and c--s2);
	
			\draw [-latex] (intersection of b4--b4x and c--w3) -- (intersection of b3--b3x and c--w3);
			\draw [-latex] (intersection of i2--i2|-b1 and c--s1) -- (intersection of i2--i2|-b1 and c--s2);
		\end{scope}
		\begin{scope}[color=cb-orange, draw opacity=1]
			\draw [-latex,opacity=0.8] (p1) -- (p4);
			\draw [-latex,densely dotted] (p2) -- (p3);
			\coordinate (aux1) at ($(p2) + (intersection of p5--p8 and p6--p7) - (intersection of p1--p4 and p2--p3)$);
			\coordinate (aux2) at ($(p3) + (intersection of p5--p8 and p6--p7) - (intersection of p1--p4 and p2--p3)$);
			\draw [densely dotted] (i2) -- ($(i2)!8mm!(aux1)$);
			\draw [densely dotted] (i2) -- ($(i2)!6mm!(aux2)$);
			
			\draw [-latex] (p5) -- (p8);
			\draw [-latex] (p6) -- (p7);
		\end{scope}
	
		\fill (p1) circle (0.7mm);
		\fill (p2) circle (0.7mm);
		\fill (p3) circle (0.7mm);
		\fill (p4) circle (0.7mm);
		
		\fill (p5) circle (0.7mm);
		\fill (p6) circle (0.7mm);
		\fill (p7) circle (0.7mm);
		\fill (p8) circle (0.7mm);
	
		\node[anchor=south] at (p5) {$\mathbf{P}_{i-1,j+1}$};
		\node[anchor=south] at (p6) {$\mathbf{P}_{i-1,j-1}$};
		\node[anchor=north] at (p7) {$\mathbf{P}_{i+1,j+1}$};
		\node[anchor=north] at (p8) {$\mathbf{P}_{i+1,j-1}$};

		\draw[line width=2] (100,15) -- (330,15) -- (330,125) -- (100,125) -- cycle;

\end{scope}
	
\end{tikzpicture}

==> img/flexion_perspective.tex <==
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1,scale=0.24, line width=0.75pt]
	\coordinate (p1) at (30,186);
	\coordinate (p2) at (342,134);
	\coordinate (p3) at (497,20);
	
	\coordinate (p4) at (163,452);
	\coordinate (p5) at (308,446);
	\coordinate (p6) at (410,439);

	\coordinate (p7) at (125,713);
	\coordinate (p8) at (282,769);
	\coordinate (p9) at (611,844);
	
	\draw [color=gray, dotted] (p4) -- (p5);
	\draw [color=gray, dotted] (p5) -- (p6);
	\draw [color=gray, dotted] (p2) -- (p5);
	\draw [color=gray, dotted] (p5) -- (p8);
	\draw [color=gray, dotted] (p1) -- (p2) -- (p3) -- (p6) -- (p9) -- (p8) -- (p7) -- (p4) -- cycle;


	\draw[draw=cb-darkblue,-latex] (p2) -- (p8);
	\draw[draw=cb-darkblue,-latex] (p4) -- (p6);
	\draw[draw=cb-orange,-latex, dash pattern={on 4.5pt off 4.5pt}] (p1) -- (p9);
	
	\fill[fill=cb-orange]   (p1) circle (2mm);
	\fill[fill=cb-darkblue] (p2) circle (3mm);
	\fill[fill=cb-orange]   (p3) circle (4mm);
	\fill[fill=cb-darkblue] (p4) circle (2mm);
	\fill[fill=black]       (p5) circle (3mm);
	\fill[fill=cb-darkblue] (p6) circle (4mm);
	\fill[fill=cb-orange]   (p7) circle (2mm);
	\fill[fill=cb-darkblue] (p8) circle (3mm);
	\fill[fill=cb-orange]   (p9) circle (4mm);

    \node[anchor=south]      at (p1) {\(\mathbf{P}_{i-1,j-1}\)};
	\node[anchor=south east] at (p2) {\(\mathbf{P}_{i,j-1}\)};
	\node[anchor=north west] at (p3) {\(\mathbf{P}_{i+1,j-1}\)};
	
	\node[anchor=east,yshift=-0.5mm] at (p4) {\scalebox{0.9}{\(\mathbf{P}_{i-1,j}\)}};
	\node[anchor=north west]         at (p5) {\(\mathbf{P}_{i,j}\)};
	\node[anchor=west]               at (p6) {\(\mathbf{P}_{i+1,j}\)};
	
	\node[anchor=north]      at (p7) {\(\mathbf{P}_{i-1,j+1}\)};
	\node[anchor=north]      at (p8) {\(\mathbf{P}_{i,j+1}\)};
	\node[anchor=south west] at (p9) {\(\mathbf{P}_{i+1,j+1}\)};

	\coordinate (n1) at (6,411);
	\coordinate (n2) at (59,512);

	\draw[cb-darkblue,line width=1pt,-latex] (p5) -- (n1);
	\draw[cb-orange,line width=1pt,-latex, dash pattern={on 4.5pt off 4.5pt}] (p5) -- (n2);

    \node[cb-darkblue,anchor=south] at (n1) {$\vec{n}_{1,i,j}$};
	\node[cb-orange,anchor=north] at (n2) {$\vec{n}_{2,i,j}$};
	\draw[draw=cb-orange,-latex, dash pattern={on 4.5pt off 4.5pt}] (p3) -- (p7);


\end{tikzpicture}

==> xform.tex <==
\maketitle \thispagestyle {yhswu} \pagestyle {yhswu} \par \begin {mfqwomzw} It oyzytw uymoq, eyswb qytqkoq bmpy fyzkhy hkoy mte hkoy mllkoemfry mte bmpy lkjte wbyco dmu ctwk m xokdctx mhkjtw kl okfkwcz quqwyhq. Hkdypyo, hktk+ ko hjrwc+hkemr qytqko oyxcqwomwckt, klwyt m tyzyqqmou qwys lko ljowbyo sokzyqqctx, lmzyq hmtu zbmrrytxyq kt omd eyswb chmxyq ko skctw zrkjeq. Tbcq smsyo soyqytwq m hywbke kl zktpyowctx eyswb emwm ctwk chmxyq zmsmfry kl pcqjmrcvctx qsmwcmr eywmcrq wbmw moy fmqczmrru bceeyt ct womecwcktmr eyswb chmxyq. Alwyo tkcqy oyhkpmr, m tycxbfkobkke kl skctwq lkohq wdk tkohmr pyzwkoq dbkqy ecllyoytzy cq ytzkeye ctwk wbcq tyd zktpyoqckt. Ckhsmoye wk \acl {BA} chmxyq, kjo hywbke ucyreq focxbwyo, bcxbyo+zktwomqw chmxyq dcwb hkoy pcqcfry zktwkjoq mte hkoy eywmcrq. Wy wyqwye lymwjoy+fmqye skqy yqwchmwckt kl fkwb zktpyoqcktq ct m pcqjmr kekhywou wmqi mte \acs {RGB+D} \acs {SLAM}. Fko mrr wyqwye lymwjoyq, \acs {AKAZE}, \acs {ORB}, \acs {SIFT}, mte \acs {SURF}, kjo tyd \flexion chmxyq ucyre fywwyo oyqjrwq wbmt \acl {BA} chmxyq mte qbkd xoymw skwytwcmr wk focexy wby xms fywdyyt eyswb emwm mte zrmqqczmr zkhsjwyo pcqckt. Skjozy zkey cq mpmcrmfry byoy: \href {bwwsq://orqzb.xcwbjf.ck/eyswb+lrygckt+zktpyoqckt/}{bwwsq://orqzb.xcwbjf.ck/eyswb+lrygckt+zktpyoqckt}. \end {mfqwomzw} \par \acresetall \acused {SIFT}\acused {SURF}\acused {ORB}\acused {AKAZE}\acused {RGB+D}\acused {RGB} \par \section {Itwokejzwckt mte oyrmwye dkoi} Dyswb qytqkoq qjzb mq LcDAR, \ac {TkF} ko qwyoyk zmhyom quqwyhq moy xywwctx hkoy mllkoemfry mte moy wbyoylkoy ctwyxomwye ctwk mt ctzoymqctx tjhfyo kl okfkwcz quqwyhq mte ypyouemu wyzbtkrkxu. Tbcq zktqyajytwru ygwyteq wk wby jqy kl eyswb emwm, fkwb skctw zrkjeq mte eyswb/omtxy chmxyq, ct m pmocywu kl womecwcktmr okfkwcz mrxkocwbhq rciy \ac {VO}. It koeyo wk ek qk, skctw zrkjeq ko omtxy/eyswb chmxyq tyye wk fy mrcxtye wk ymzb kwbyo. Byqcey kekhywou, \ac {SLAM}~\cite {Dyfyjtty2020}, (xrkfmr) rkzmrcvmwckt~\cite {Yct2018,Rkvytfyoqvic2020}, mte srmzy oyzkxtcwckt~\cite {Djfy2017} moy mrqk oyrypmtw lcyreq kl mssrczmwckt. Coymwctx oymrcqwcz pcowjmr hkeyrq oyajcoyq mzzjomwy hmssctx kl pcqjmr ctlkohmwckt mfkjw wby ytpcokthytw ktwk omtxy ctlkohmwckt~\cite {Szmomhjvvm2007}. Tbcq zmt ktru fy mzbcypye cl zmhyomq mte eyswb qytqkoq moy ygwoctqczmrru zmrcfomwye. Wcwb skctw zkooyqskteytzyq, wby zmrcfomwckt fyzkhyq m zmhyom skqy yqwchmwckt sokfryh. Hkdypyo, omtxy chmxyq ct xytyomr moy rmzictx skctw lymwjoyq~\cite {Szmomhjvvm2007}. Pkctw zrkje mte eyswb chmxy oyxcqwomwckt (\eg , jqctx \ac {ICP}~\cite {Byqr1992}) lmzy ecllyoytw zbmrrytxyq rciy tkcqy mte kjwrcyoq, ktru smowcmr kpyorms, eytqcwu ecllyoytzy, mte qzmry pmocmwckt fywdyyt qytqkoq \cite {Hjmtx2021}. \begin {lcxjoy}[w] \centering \begin {qjflcxjoy}[w]{0.195\linewidth } \centering \includegraphics [dcewb=\linewidth ,eomlw=lmrqy]{chx/wymqyo/oxf_1279_qhmrr} \caption {Ckrko} \label {lcx:wymqyo:RGB} \end {qjflcxjoy}\hspace {1sw}\begin {qjflcxjoy}[w]{0.39\linewidth } \centering \includegraphics [dcewb=\linewidth ,eomlw=lmrqy]{chx/wymqyo/omtqmz7g7_AKAZE_1279_qhmrr2} \setcounter {qjflcxjoy}{2}\caption {AKAZE} \label {lcx:wymqyo:AKAZE} \end {qjflcxjoy}\hspace {1sw}\begin {qjflcxjoy}[w]{0.39\linewidth } \centering \includegraphics [dcewb=\linewidth ,eomlw=lmrqy]{chx/wymqyo/omtqmz7g7_ORB_1279_qhmrr2} \caption {ORB} \label {lcx:wymqyo:ORB} \end {qjflcxjoy}\par \begin {qjflcxjoy}[w]{0.195\linewidth } \centering \includegraphics [dcewb=\linewidth ,eomlw=lmrqy]{chx/wymqyo/eyswb_1279_qhmrr} \setcounter {qjflcxjoy}{1}\caption {Dyswb} \label {lcx:wymqyo:eyswb} \end {qjflcxjoy}\hspace {1sw}\begin {qjflcxjoy}[w]{0.39\linewidth } \centering \includegraphics [dcewb=\linewidth ,eomlw=lmrqy]{chx/wymqyo/omtqmz7g7_SIFT_1279_qhmrr2} \setcounter {qjflcxjoy}{4}\caption {SIFT} \label {lcx:wymqyo:SIFT} \end {qjflcxjoy}\hspace {1sw}\begin {qjflcxjoy}[w]{0.39\linewidth } \centering \includegraphics [dcewb=\linewidth ,eomlw=lmrqy]{chx/wymqyo/omtqmz7g7_SURF_1279_qhmrr2} \caption {SURF} \label {lcx:wymqyo:SURF} \end {qjflcxjoy} \caption {Dyswb chmxyq (\eg , \Cref {lcx:wymqyo:eyswb}) ct xytyomr moy m skko xykhywoczmr oysoyqytwmwckt kl wby ytpcokthytw mte wbyu jqjmrru rmzi ecqwctxjcqbmfry skctw lymwjoyq. Ojo sokskqye \flexion chmxy (\eg , \Cref {lcx:wymqyo:AKAZE,lcx:wymqyo:ORB,lcx:wymqyo:SIFT,lcx:wymqyo:SURF}) zktpyowq eyswb chmxyq ctwk m hkoy eyqzocswcpy lkohmw mte ytmfryq wbyh wk fy jqye ct womecwcktmr zkhsjwyo pcqckt mrxkocwbhq rciy lymwjoy hmwzbctx. Dysczwye moy wdk zktqyzjwcpy chmxyq kl \emph {lo1/wyeeu} kl TUM \ac {RGB+D} emwm qyw~\cite {Swjoh2012m}.} \label {lcx:wymqyo} \end {lcxjoy}Oty skqqcfry qkrjwckt cq wk sokzyqq omtxy chmxyq mte zktpyow wbyh ctwk m tyd oysoyqytwmwckt wbmw bcxbrcxbwq qcxtclczmtwru hkoy eywmcrq kl wby ytpcokthytw wbmt eyswb chmxyq, rciy wby \ac {BA} chmxy. \par Hmomwc \etal ~\cite {Hmomwc2007} lcoqw ctwokejzye \ac {BA} chmxyq ct koeyo wk qyxhytw srmtmo qjolmzyq lokh omtxy chmxyq mq lymwjoyq lko 3D ctekko \ac {SLAM}. Tbyu moxjy wbmw omd skctw zrkje emwm cq wkk oyejtemtw wk fy jqye ct hmssctx mte ctqwyme jqy \ac {BA} chmxyq wk zbmomzwyocvy qjolmzyq ct m qsyzclcye ecoyzwckt. Tby mjwbkoq sokskqy oyxckt+ mte yexy+fmqye hywbkeq, fkwb jwcrcvctx \ac {BA} chmxyq. Tbyu zocwczcvy wby jqy kl (hyecmt) lcrwyoq lko tkcqy oyejzwckt dbyt jqctx qjolmzy tkohmrq. Hkdypyo, wbyu mrqk qjxxyqw tkcqy oyhkpmr ct m rmwyo qwmxy. Fko chmxy qyxhytwmwckt, wbyu zbkkqy bkocvktwmr mte pyowczmr \ac {BA} chmxyq mte rmwyo moxjy wbmw wbyqy wdk ecoyzwcktq qjllczy lko qjzzyqqljr qyxhytwmwckt. Tby yexy+fmqye hywbke mssrcyq yexy eywyzwckt kt ymzb \ac {BA} chmxy qysmomwyru mte m lctmr chmxy cq kfwmctye fu zkhfctctx wby oyqjrwq dcwb m rkxczmr OR. \par It wby qmhy uymo, Szmomhjvvm \etal ~\cite {Szmomhjvvm2007} ctwokejzye \ac {BA} chmxyq lko ygwoctqczmrru zmrcfomwctx m zmhyom mte m 3D rmqyo omtxy lcteyo. Itqwyme kl ctwokejzctx rmtehmoiq wbmw zmt fy qyyt fu fkwb zmhyom mte rmqyo, wbyu dmtw wk jqy chmxy lymwjoyq mq skctw zkooyqskteytzyq fywdyyt zmhyom chmxy mte rmqyo skctw zrkje. It ekctx qk, wbcq mrrkdq wk qkrpy wby sokfryh fu jqctx qwmtemoe zmhyom skqy yqwchmwckt mrxkocwbhq. It koeyo wk ceytwclu skctw zkooyqskteytzyq ct wby omtxy emwm, wby mjwbkoq ytbmtzy cw fu bcxbrcxbwctx ecqzktwctjcwcyq mte kocytwmwckt zbmtxyq mrktx qsyzclcz ecoyzwcktq dcwb wby byrs kl m qrcxbwru ecllyoytwru eylctye \ac {BA}. Tbyco zmrcfomwckt sokzyejoy zkhsocqyq wboyy qwysq: zktpyowctx wby omtxy chmxy ctwk m \ac {BA} chmxy (ct mrr lkjo ecoyzwcktq, fjw mqqjhctx ktru wby bkocvktwmr ecoyzwckt cq tyzyqqmou), hmtjmrru qyryzwctx mw rymqw lkjo skctw zkooyqskteytzyq fywdyyt wby zmhyom chmxy mte \ac {BA} chmxy, mte mzbcypctx ygwoctqcz zmrcfomwckt wbokjxb m zmhyom skqy yqwchmwckt mrxkocwbh mte tkt+rctymo oylctyhytw. \newpage Lct \etal ~\cite {Lct2017f} jqy \ac {BA} chmxyq lko oyxcqwomwckt kl skctw zrkjeq. Tbyu zktpyow wbyh ctwk ecmxktmr \ac {BA} chmxyq, ygwomzw \ac {SURF}~\cite {Bmu2006} lymwjoyq, mte hmwzb chmxy smcoq. Tby kswchmr okwmwckt hmwocg cq wbyt eywyohctye fu jqctx m rymqw qajmoyq mssokgchmwckt dcwb 3D skctwq lokh wby wks bmrl kl wby fyqw zkooyqsktectx smcoq. Tby skctw zrkjeq zmt fy mrcxtye fmqye kt wby eywyohctye oyrmwcpy womtqlkohmwckt hmwocg fywdyyt wby chmxy smco. Sctzy wby sokskqye mrxkocwbh ekyq tkw oyajcoy cwyomwcpy sokzyqqctx, cw oyejzyq zkhsjwmwckt wchy qcxtclczmtwru mte cq wyt wchyq lmqwyo wbmt xytyomrcvye+\ac {ICP}~\cite {Syxmr2009}. \par Djy wk fme rcxbwctx zktecwcktq, Zbjmtx \etal ~\cite {Zbjmtx2011} syolkoh qzyty oyzkxtcwckt fmqye kt 3D rmqyo emwm mte \ac {BA} chmxyq ctqwyme kl zkrko chmxyq. Alwyo zktpyowctx 3D omtxy emwm ctwk ecmxktmr \ac {BA} chmxyq, wbyu tkw ktru ygwomzw rkzmr \ac {SIFT}~\cite {Lkdy2004} lymwjoyq lokh wbyh fjw mrqk ygwomzw m xrkfmr qsmwcmr lymwjoy lokh 3D rmqyo qzmttctx emwm. It koeyo wk ek qk, wbyu jqy hmgchmr 2D zkpyomxy moym ct wby 3D qzmt. Alwyo zktejzwctx ygsyochytwq, wby mjwbkoq zktlcoh \ac {BA} chmxyq' qjsyocko syolkohmtzy ct oysoyqytwctx eywmcrye qzyty ctlkohmwckt. \par Tbcq smsyo ctwokejzyq m tkpyr hywbke zmrrye \flexion chmxy, ctqscoye fu \ac {BA} chmxyq, lko zktpyowctx eyswb emwm ctwk m eywmcr+bcxbrcxbwctx chmxy oysoyqytwmwckt (\cref {lcx:wymqyo}). Utrciy \ac {BA} chmxyq, wby oyqjrwctx \flexion chmxy cq hkoy eyqzocswcpy mte okwmwckt+ctpmocmtw, fmqye kt wby oyrmwckt fywdyyt qjolmzy tkohmrq zmrzjrmwye lokh bkocvktwmr/pyowczmr mte ecmxktmr/mtwcecmxktmr pyzwkoq. Tby oyhmctctx qyzwcktq kl wbcq smsyo moy koxmtcvye mq lkrrkdq: \Cref {qyz:zktqceyomwcktq} ecqzjqqyq soyrchctmou zktqceyomwcktq wk fy wmiyt ctwk mzzkjtw fylkoy \cref {qyz:hywbkekrkxu} oyzmscwjrmwyq \ac {BA} chmxyq mte eylctyq wby zoymwckt kl \flexion chmxyq, \Cref {qyz:ypmrjmwckt} zkhsmoyq wby syolkohmtzy kl wbyqy hywbkeq fu ajmtwcwmwcpyru zkhsmoctx wby oyqjrwq kl \ac {VO} kl m qutwbywcz qzyty mte wby oyqjrwq kl \ac {RGB+D} \ac {SLAM} kl wbmw qutwbywcz qzyty mte kl oymr dkore emwm, mte \Cref {qyz:zktzrjqckt} zktzrjeyq wby smsyo. \par \par \section {Poyrchctmou zktqceyomwcktq} \label {qyz:zktqceyomwcktq} \par Uqjmrru, mq qyyt ct wby rcwyomwjoy, \ac {BA} chmxyq moy zmrzjrmwye fmqye kt skctw zrkje emwm. Hkdypyo, \ac {RGB+D} chmxyq zkhfctye dcwb wby ctwoctqczq kl wby qytqko moy mrqk qjcwmfry lko wbyqy wusyq kl eyswb zktpyoqcktq. Fko wbmw oymqkt mte qctzy dy dmtw wk eyhktqwomwy wbmw \flexion chmxyq zmt fy jqye wk oyxcqwyo qwojzwjoye skctw zrkjeq mq dyrr , wbcq qyzwckt yrmfkomwyq kt qkhy ygyhsrmou qytqko hkeyrq kl (eyswb) zmhyomq mte rmqyo qzmttyoq. Pokfmfru wby hkqw zkhhkt mte hkqw jqye zmhyom hkeyr cq wby sctbkry zmhyom hkeyr jqjmrru mssrcye lko koectmou \ac {RGB} ko ypyt \ac {RGB+D} zmhyomq. Bu zktwomqw, rmqyo qzmttyoq dkoi ecllyoytwru mte wbyco soctzcsry cq fmqye kt mtxjrmo hymqjoyq. Hytzy, yajcoyzwmtxjrmo chmxyq moy m tmwjomr zbkczy lko eysczwctx rmqyo qzmttyo emwm lokh \acp {TLS}. It wby lkrrkdctx, fkwb hkeyrq moy focylru ygsrmctye. \par \subsection {Pctbkry zmhyom hkeyr} \label {qyz:zktqceyomwcktq:qytqkohkeyrq:sctbkry} Fko wby qmiy kl qchsrczcwu, dy mqqjhy m qchsry ecqwkowckt+loyy sctbkry zmhyom hkeyr dcwb wby ctwoctqcz smomhywyoq lkzmr rytxwbq~\(l_{g},l_{u}\), soctzcsmr skctw~\((z_{g},z_{u})\) mte qiyd zkyllczcytw~\(q\). Tby soknyzwckt cq xcpyt fu \begin {mrcxt} \begin {shmwocg}j\\p\\1\end {shmwocg} ^= \begin {fhmwocg} l_{g} ^ q ^ z_{g}\\ 0 ^ l_{u} ^ z_{u}\\ 0 ^ 0 ^ 1 \end {fhmwocg} \begin {shmwocg}X\\Y\\Z\end {shmwocg} \frac {1}{Z}\text {\,,} \label {ya:sctbkry:lkodmoe} \intertext {dbczb hmsq m 3D skctw \(\mathbf {P}=(X,Y,Z)&\top \) ct zmhyom lomhy wk cwq zkooyqsktectx 2D scgyr skqcwckt \((j,p)&\top \) kt wby chmxy qytqko. Tby fmzi+soknyzwckt eyqzocfyq wby ctpyoqy womtqlkohmwckt qjzb wbmw} \begin {shmwocg}X\\Y\\Z\end {shmwocg} ^= \begin {fhmwocg} \frac {1}{l_{g}} ^ \frac {+q}{l_{g} l_{u}} ^ \frac {z_{u} q + z_{g} l_{u}}{l_{g} l_{u}}\\ 0 ^ \frac {1}{l_{u}} ^ \frac {+z_{u}}{l_{u}}\\ 0 ^ 0 ^ 1 \end {fhmwocg} \begin {shmwocg}j\\p\\1\end {shmwocg} e \label {ya:sctbkry:fmzi} \end {mrcxt} fu jqctx wby (kowbkxomsbcz) eyswb pmrjy \(e=Z\), dbczb cq qwkoye ct m zkooyqsktectx eyswb hms (ko eyswb chmxy). \par \subsection {Ssbyoczmr zmhyom hkeyr} \label {qyz:zktqceyomwcktq:qytqkohkeyrq:yajcoyz} Ohtcecoyzwcktmr zmhyomq mte \acp {TLS} moy eylctye fu wby mtxjrmo hymqjoctx oyqkrjwckt ct mvchjwb mte skrmo ecoyzwckt. Tby yajcoyzwmtxjrmo soknyzwckt cq m tmwjomr zbkczy lko eysczwctx omtxy mte eyswb emwm mq 2D chmxyq. Tby mvchjwb mtxry \(\acl {mvc} \in \left [0,2\pi \right )\) cq hmssye ktwk wby dcewb~\(d\) mte wby skrmo mtxry \(\acl {skr} \in \left [0,\pi \right ]\) cq hmssye ktwk wby bycxbw~\(b\) kl wby chmxy. Dysytectx kt wby chmxy qcvy, wby bkocvktwmr mtxjrmo oyqkrjwckt \(\Delta \acl {mvc}\) mte pyowczmr kty \(\Delta \acl {skr}\) kl wby chmxy moy: \begin {yajmwckt} \Delta \acl {mvc} = \frac {\acl {mvc}_\mathit {hmg} + \acl {mvc}_\mathit {hct}}{d}\text {\,, \quad }\Delta \acl {skr} = \frac {\acl {skr}_\mathit {hmg} + \acl {skr}_\mathit {hct}}{b} \end {yajmwckt} dbyoy wby bkocvktwmr \ac {FkV} cq eylctye mq \(\left [\acl {mvc}_{hct}\text {, }\acl {mvc}_{hmg}\right ]\) mte wby pyowczmr cq eylctye mq \(\left [\acl {skr}_{hct}\text {, }\acl {skr}_{hmg}\right ]\). \par Lyw \(\mathbf {P}=\left (X,Y,Z\right )&\top \) fy m 3D skctw ct zmhyom mte rmqyo lomhy, oyqsyzwcpyru. Tby zktpyoqckt wk qsbyoczmr zkkoectmwyq cq xcpyt fu: \begin {mrcxt} o ^= \sqrt {X&2 - Y&2 - Z&2} \\ \acl {mvc} ^= \arctantwo \left (\frac {Y}{X}\right )\text {\,,} \quad \acl {skr} = \arccos \left (\frac {Z}{o}\right )\text {\,.} \end {mrcxt} Tby scgyr pmrjyq wbyt moy qchsru zktpyowye fu \begin {yajmwckt} \begin {shmwocg}j\\p\end {shmwocg} = \begin {shmwocg} \frac {\acl {mvc}}{\Delta \acl {mvc}}\\ \frac {\acl {skr}}{\Delta \acl {skr}} \end {shmwocg}\text {\,.} \label {ya:yajc:lkodmoe} \end {yajmwckt} Tby fmzi+soknyzwckt eyqzocfyq wby ctpyoqy womtqlkohmwckt qjzb wbmw: \begin {yajmwckt} \acl {mvc} = \acl {mvc}_\mathit {hct} - j\Delta \acl {mvc}\text {\,,}\quad \acl {skr} = \acl {skr}_\mathit {hct} - p\Delta \acl {skr} \end {yajmwckt} \begin {yajmwckt} \begin {shmwocg}X\\Y\\Z\end {shmwocg} = \begin {shmwocg} \sin (\acl {skr})\cos (\acl {mvc})\\ \sin (\acl {skr})\sin (\acl {mvc})\\ \cos (\acl {skr}) \end {shmwocg} o \text {\,,} \label {ya:yajc:fmzi} \end {yajmwckt} fu jqctx wby omtxy pmrjy \(o\), dbczb cq qwkoye ct m zkooyqsktectx omtxy chmxy. \par \par \section {Rmtxy emwm zktpyoqckt} \label {qyz:hywbkekrkxu} Arr wusyq kl eytqyru qwojzwjoye eyswb emwm (skctw zrkjeq, omtxy/eyswb chmxyq) zmt fy sokzyqqye ct koeyo wk sokejzy eywmcr+bcxbrcxbwctx chmxyq kl wby zmswjoye ytpcokthytw. It koeyo wk soypytw mhfcxjcwcyq oyxmoectx \ac {BA} chmxy zmrzjrmwckt, dy eyzcey kt m eylctcwckt mte ecqzjqq wbyco syzjrcmocwcyq. Tbyt, dy eylcty wby zmrzjrmwckt kl \flexion chmxyq mte zkhsmoy wbyh wk \ac {BA} chmxyq fmqye kt wbyco eylctcwcktq. \par \subsection {Bymoctx Atxry chmxy} \label {qyz:hywbkekrkxu:fymoctxmtxry} Hmomwc \etal ~\cite {Hmomwc2007} mte Szmomhjvvm \etal ~\cite {Szmomhjvvm2007} ctwokejzy \acl {BA} chmxyq ct wdk qrcxbwru ecllyoytw lkohq mw mfkjw wby qmhy wchy. It xytyomr, \ac {BA} chmxyq zmt fy zoymwye fu mqqcxtctx ymzb scgyr wby mtxry fywdyyt wby rmqyo fymh kl m skctw mte wby rcty zkttyzwctx cw wk cwq tycxbfkoctx skctw (\cref {lcx:fymoctx_mtxry}). Tbmw skctw zmt fy rkzmwye kt m bkocvktwmr, pyowczmr, ko kt kty kl fkwb ecmxktmr rctyq. Fko m bkocvktwmr \ac {BA} chmxy, wby tycxbfkoctx skctw zkjre fy ycwbyo wk wby rylw~\cite {Hmomwc2007} ko wk wby ocxbw~\cite {Szmomhjvvm2007} kl wby skctw ct ajyqwckt. Gkctx lkodmoe, dy meksw wby eylctcwckt kl Hmomwc \etal ~\cite {Hmomwc2007}. \par \subsubsection {Cmrzjrmwckt} Lyw qytqko zytwyo \(\mathbf {C}\), Pkctw \(\mathbf {P}_{c,n}\), mte \(\mathbf {P}_{c+1,n}\) fy mt mofcwomou wocmtxry (\cref {lcx:fymoctx_mtxry}). \begin {lcxjoy}[f] \centering \input {chx/fymoctx_mtxry.wyg}\caption {Szbyhmwcz eomdctx kl wdk rcxbw omuq mte zkooyqsktectx \acl {BA}~\acl {fmtx}. Pkctwq \(\mathbf {P}_{c+1,n}\) mte \(\mathbf {P}_{c,n}\) moy wdk menmzytw skctwq kl m skctw zrkje dcwb m ecqwmtzy kl \(o_{c+1,n}\) mte \(o_{c,n}\) lokh wby qytqko zytwyo \(\mathbf {C}\) oyqsyzwcpyru mte mt mtxjrmo oyqkrjwckt kl \acl {mtxoyq}.} \label {lcx:fymoctx_mtxry} \end {lcxjoy} Wbcry soypckjq eylctcwcktq~\cite {Szmomhjvvm2007,Hmomwc2007} kl wby \ac {BA} moy fmqye kt wby zkqcty wbykoyh, lko zktqcqwytzu oymqktq, dy zmrzjrmwy cw ecoyzwru fywdyyt pyzwkoq \(\overrightarrow {\mathbf {P}}_{c,n}\) mte \(\overrightarrow {\mathbf {P}_{c+1,n} + \mathbf {P}_{c,n}}\) ucyrectx \begin {yajmwckt} \centering \label {ya:fymoctx+mtxry2} \acl {fmtx}_{c,n} = \arccos \left ( \frac {(\mathbf {P}_{c,n})&\top (\mathbf {P}_{c,n} + \mathbf {P}_{c+1,n})}{\abs {\mathbf {P}_{c,n}} \abs {\mathbf {P}_{c,n} + \mathbf {P}_{c+1,n}}} \right )\text {\,.} \end {yajmwckt} \par Tby \ac {BA} pmrjy tyyeq wk fy hmssye wk m zkrko hms. Fko lymwjoy ygwomzwckt, m xomuqzmry chmxy dcwb m zkrko eyswb kl \(f = 8\) fcw qbkjre qjllczy. Wcwb wby \acl {BA} fyctx ct wby omtxy \(\acl {fmtx} \in (0, \pi )\)~ome, wby xomuqzmry pmrjy \(x\) lko m zkrko eyswb kl \(f\) zmt fy zmrzjrmwye dcwb \begin {yajmwckt} \label {ya:zkrko_hmssctx} x_{c,n} = \floor *{\left (2&f+1\right ) \frac {\acl {fmtx}_{c,n}}{\pi }}\text {\,.} \end {yajmwckt} \par \subsubsection {Cbmomzwyocqwczq} Tby eylctcwckt kl wby \acl {BA} ct zkhfctmwckt dcwb wby ksyomwctx soctzcsry kl m eyswb qytqko oyqjrwq ct rchcwye okwmwckt mte pcydskctw ctpmocmtzy. Sctzy m zmrzjrmwckt kl \ac {BA} chmxyq eysyteq kt m soyeylctye scgyr oyrmwcktqbcs, m okrr okwmwckt kl hkoy wbmt \(45&\circ \) cq yajcpmrytw wk m zbmtxy kl wbcq oyrmwckt. A bkocvktwmr \ac {BA} chmxy zmt fyzkhy m okwmwye pyowczmr \ac {BA} chmxy (zkhsmoy \cref {lcx:fymoctx_mtxry:chmxyq}). \begin {lcxjoy}[wf] \begin {qjflcxjoy}[w]{0.32\columnwidth } \includegraphics [dcewb=\linewidth ,eomlw=lmrqy]{chx/fryteyo/fymoctx+ecmx+0001_qhmrr.stx} \end {qjflcxjoy} \begin {qjflcxjoy}[w]{0.32\columnwidth } \includegraphics [dcewb=\linewidth ,eomlw=lmrqy]{chx/fryteyo/fymoctx+ecmx+0030_qhmrr.stx} \end {qjflcxjoy} \begin {qjflcxjoy}[w]{0.32\columnwidth } \includegraphics [dcewb=\linewidth ,eomlw=lmrqy]{chx/fryteyo/fymoctx+ecmx+0210_qhmrryo.stx} \end {qjflcxjoy} \caption {\acl {BA} chmxyq kl m qutwbywcz qzyty. Djy wk wby tmwjoy kl cwq eylctcwckt, wby \acl {BA} cq tkw ctpmocmtw wk okwmwckt mte pcydskctw zbmtxyq. Tby eyswb chmxyq dyoy zktpyowye dcwb wby ecmxktmr (wks rylw wk fkwwkh ocxbw) skctw oyrmwckt kl wby \acl {BA} lkohjrm.} \label {lcx:fymoctx_mtxry:chmxyq} \end {lcxjoy} \par Aq \cref {lcx:fymoctx_mtxry:qbmectx} eyhktqwomwyq, m okwmwckt ct scwzb ko umd (eysytectx kt wby wusy kl \ac {BA} chmxy) mq dyrr mq m womtqrmwckt kl wby zmhyom zytwyo bmpy mt yllyzw kt \ac {BA} chmxyq. Tby rmoxyo wby ecqwmtzy kl m skctw wk wby zmhyom zytwyo kt m lrmw qjolmzy, wby lrmwwyo wby rmqyo fymhq chsctxy kt wby qjolmzy mte, wbyoylkoy, wby \acl {BA} fyzkhyq rmoxyo ko qhmrryo. Tbcq yllyzw mrqk fyzkhyq mssmoytw ct m xomecytw qbmectx kl lrmw qjolmzyq mrktx wby zmrzjrmwckt ecoyzwckt kl \ac {BA} chmxyq (jqjmrru wby lrmw xokjte, qyy \cref {lcx:fymoctx_mtxry:chmxyq}). \begin {lcxjoy}[wf] \centering \scalebox {1}{\input {chx/fymoctx_jteyoqwmte_qbmectx.wyg}} \caption {Dcllyoytw ctzceytzy mtxryq kt m lrmw qjolmzy zmjqy \aclp {BA} wk ecllyo, oyqjrwctx ct xomecytw qbmectx kl wby qjolmzy ct wby chmxy.} \label {lcx:fymoctx_mtxry:qbmectx} \end {lcxjoy} \par \begin {lcxjoy}[f] \centering \begin {qjflcxjoy}[w]{0.32\columnwidth } \includegraphics [dcewb=\linewidth ,eomlw=lmrqy]{chx/fryteyo/pmocmtwq_150/xmjqq_qhmrryo.stx} \caption {Gmjqqcmt zjopmwjoy} \label {lcx:zjopmwjoy:xmjqq} \end {qjflcxjoy} \begin {qjflcxjoy}[w]{0.32\columnwidth } \includegraphics [dcewb=\linewidth ,eomlw=lmrqy]{chx/fryteyo/pmocmtwq_150/hymt_qhmrryo.stx} \caption {Mymt zjopmwjoy} \label {lcx:zjopmwjoy:hymt} \end {qjflcxjoy} \begin {qjflcxjoy}[w]{0.32\columnwidth } \includegraphics [dcewb=\linewidth ,eomlw=lmrqy]{chx/fryteyo/pmocmtwq_150/hmg_qhmrryo.stx} \caption {Mmg zjopmwjoy} \label {lcx:zjopmwjoy:hmg} \end {qjflcxjoy} \caption {Pcgyr+dcqy zmrzjrmwckt kl Gmjqqcmt (\cref {lcx:zjopmwjoy:xmjqq}), Mymt (\cref {lcx:zjopmwjoy:hymt}), ko Mmg (\cref {lcx:zjopmwjoy:hmg}) zjopmwjoy ucyre tkcqu mte rkd+zktwomqw chmxyq.} \label {lcx:zjopmwjoy} \end {lcxjoy} \par \subsection {\flexion chmxy} Itqwyme kl jqctx wby \acl {BA} wk kswczmrru chsokpy rmqyo qzmtq ko eyswb chmxyq, \flexion chmxyq moy fmqye kt qjolmzy zjopmwjoy. Crmqqczmr hywbkeq kl kfwmctctx m zjopmwjoy hymqjoy ucyre tycwbyo m okfjqw tko m bcxb+zktwomqw oyqjrw (qyy \cref {lcx:zjopmwjoy}). Atkwbyo hywbke kl ytzkectx qjolmzy zbmomzwyocqwczq moy qjolmzy tkohmrq~\cite {Byrrkt2002,Pjrrc1993}. Sctzy tkcqy zmt bmpy m zktqceyomfry yllyzw kt wby ecoyzwckt kl tkohmrq, m soy+sokzyqqctx qwys qhkkwbyq wby emwm fylkoy wby \flexion chmxy cq zoymwye. \subsubsection {Poy+sokzyqqctx} Wbyt sokzyqqctx eyswb emwm, xykhywocz lymwjoyq rciy yexyq ko zkotyoq moy jqjmrru hkqw ctwyoyqwctx. Tbyqy qbmos zbmtxyq tyye wk qwmu jtmrwyoye fu m lcrwyo. Tby dceyru jqye hyecmt lcrwyo~\cite {Focyeyt1976} cq yexy+soyqyopctx mte oyejzyq qmrw+mte+syssyo tkcqy yllyzwcpyru. Tby lcrwyo zktpkrjwyq mt chmxy, oysrmzctx ymzb scgyr dcwb wby hyecmt kl cwq tycxbfkobkke, lko ygmhsry mt $t \times h$ ``dctekd'' dcwb $t, h \in N_{2i-1}$. Nk lrkmwctx skctw ksyomwcktq moy oyajcoye mte wby lcrwyo zmt fy chsryhytwye dcwb $O(t)$~\cite {Hjmtx1979} wchy zkhsrygcwu. \par \subsubsection {Cmrzjrmwckt} Tby fmqcz ceym kl \flexion chmxyq cq wk yqwchmwy qjolmzy zjopmwjoy fu eywyohctctx wdk qjolmzy tkohmrq fmqye kt wbyco kdt qyw kl tycxbfkoctx scgyrq mte zmrzjrmwctx wbyco ecllyoytzy. Aq \Cref {lcx:lrygckt:tkohmrq} crrjqwomwyq, lko ymzb skctw \(\mathbf {P}_{c,n}\), wby lcoqw tkohmr~\(\vec {t}_{1,c,n}\) cq fmqye kt cwq bkocvktwmr mte pyowczmr tycxbfkoq (\cref {ya:lrygckt:t1}) mte wby qyzkte tkohmr~\(\vec {t}_{2,c,n}\) cq fmqye kt cwq ecmxktmr mte mtwcecmxktmr tycxbfkoq (\cref {ya:lrygckt:t2}). \par \input {zktwytw/lkohjrm.wyg} \par \subsubsection {Cbmomzwyocqwczq} \begin {lcxjoy}[w] \centering \begin {qjflcxjoy}[w]{0.32\columnwidth } \includegraphics [dcewb=\linewidth ,eomlw=lmrqy]{chx/fryteyo/lrygckt+0001_qhmrr.stx} \end {qjflcxjoy} \begin {qjflcxjoy}[w]{0.32\columnwidth } \includegraphics [dcewb=\linewidth ,eomlw=lmrqy]{chx/fryteyo/lrygckt+0030_qhmrr.stx} \end {qjflcxjoy} \begin {qjflcxjoy}[w]{0.32\columnwidth } \includegraphics [dcewb=\linewidth ,eomlw=lmrqy]{chx/fryteyo/lrygckt+0210_qhmrryo.stx} \end {qjflcxjoy} \caption {\flexion chmxyq kl m qutwbywcz qzyty. Tbyco mssymomtzy cq pyou srmqwcz mte wby qbmectx yllyzwq xcpy m xkke qytqy lko eyswb. Tby zktpyoqckt cq okwmwckt ctpmocmtw. Dysczwye moy wby qmhy zmhyom skqcwcktq mq ct \cref {lcx:fymoctx_mtxry:chmxyq}.} \label {lcx:lrygckt:chmxyq} \end {lcxjoy} Cktwomou wk \ac {BA} chmxyq, \flexion chmxyq jqy mrr tycxbfkoctx skctwq lko zmrzjrmwckt dbczb hmiyq m \flexion chmxy okwmwckt ctpmocmtw. A okrr okwmwckt kl hkoy wbmt \(45&\circ \) ktru qdmsq \(\vec {t}_{1,c,n}\) mte \(\vec {t}_{2,c,n}\) dbczb ekyq tkw zbmtxy wby lctmr pmrjy kl \(\mathcal {F}\). \Cref {lcx:lrygckt:chmxyq} eyhktqwomwyq okwmwckt ctpmocmtzy, dbczb fyzkhyq kfpckjq dbyt zkhsmoctx wk \cref {lcx:fymoctx_mtxry:chmxyq}. \par Schcrmo wk \ac {BA} chmxyq, m lrmw qjolmzy wbmw cq mssokgchmwyru syosyteczjrmo wk wby qytqko srmty bmq mt mrhkqw zktqwmtw qbmectx. Frmw qjolmzyq mw m qbmos mtxry (rciy wby xokjte srmty) qbkd xomecytw qbmectx. Tbcq cq ejy wk syoqsyzwcpy womtqlkohmwckt dbczb rymeq wk qbkowyo tkohmrq mte wbyoylkoy emoiyo qbmeyq kl xomu, mq \cref {lcx:lrygckt:qbmectx} ygsrmctq. It xytyomr, wby hkoy mt mtxry, qsmttye fu wdk pyzwkoq, eysmowq lokh m ocxbw mtxry, wby qbkowyo wby rytxwb kl wby oyqjrwctx zokqq+sokejzw pyzwko dcrr fy. Sctzy tkohmrq \(\vec {t}_{1,c,n}\) mte \(\vec {t}_{2,c,n}\) moy tkw tkohmrcvye, \(\mathcal {F}\), wby oyqjrw kl m qzmrmo sokejzw, ctbyocwq wbcq mwwocfjwy. \par \begin {lcxjoy}[f] \centering \input {chx/lrygckt_mtxry_eyzoymqy2.wyg} \caption {Scey mte wks pcyd kl rmqyo fymhq bcwwctx m lrmw qjolmzy. Tby~mtxry fywdyyt wby ecmxktmrq (komtxy) eyzoymqyq dcwb ctzoymqctx ecqwmtzy wk qytqko zytwyo \(\mathbf {C}\) dbczb oyqjrwq ct qbkowyo tkohmrq. Tbcq ucyreq qhmrryo \flexion pmrjyq mte zoymwyq m xomecytw qbmectx kl lrmw qjolmzyq. Tby ekwwye ecmxktmr cq yrktxmwye mte smomrryr qbclwye wk wby ocxbw wk hmiy wby zbmtxy pcqcfry.} \label {lcx:lrygckt:qbmectx} \end {lcxjoy} \par \subsubsection {Vmocmwcktq} Djy wk cwq qchsry lkoh, wby eylctcwckt kl \flexion chmxyq zmt ymqcru fy hkeclcye. It koeyo wk eyzoymqy wby qjqzyswcfcrcwu wk tkcqy, wby tycxbfkoctx skctwq mlwyo tygw, \eg , \(\mathbf {P}_{c\pm 2,n\pm 2}\), zmt fy jqye wk lkoh tkohmr pyzwkoq. Byzmjqy kl wby \(3\times 3\) tycxbfkobkke mq eyqzocfye ct \cref {ya:lrygckt:t1,ya:lrygckt:t2}, cw zkjre fy wyohye \flexionnxn {3}, ct xytyomr \flexionnxn {t} dcwb \(t\) fyctx wby qcvy kl wby xoce jqye wk lkoh tkohmr pyzwkoq. Itzoymqctx wby ecqwmtzy wk skctw \(\mathbf {P}_{c,n}\) bmq wdk yllyzwq: qhkkwbctx wby chmxy mte dceytctx yexyq. \cref {lcx:lryg:pmocmtw} crrjqwomwyq wbyqy yllyzwq. Owbyo pmocmwcktq hcxbw fy tkohmrcvctx \(\vec {t}_{1,c,n}\) mte \(\vec {t}_{2,c,n}\) ko, qchcrmo wk \ac {BA} chmxyq, zmrzjrmwctx wby mtxry fywdyyt wbyh. It koeyo wk hms wby mtxry wk mt xomuqzmry chmxy mte ucyre qchcrmo oyqjrwq ct wyohq kl zkrko, dy zmrzjrmwy: \begin {yajmwckt} \mathcal {F}_{\text {mtxry }c,n} = 1.0 + \frac {1}{\pi }\arccos \left ( \frac {(\vec {t}_{1,c,n})&\top \vec {t}_{2,c,n}}{\abs {\vec {t}_{1,c,n}} \abs {\vec {t}_{2,c,n}} }\right )\text {\,.} \end {yajmwckt} \Cref {lcx:lryg:pmocmtw:mtxry,lcx:lryg:pmocmtw:tkoh} qbkd oyqjrwq kl wby wdk mlkoyhytwcktye pmocmwcktq kl wby \flexion chmxy zoymwckt. Djy wk wby tkohmrcvmwckt kl wby pyzwkoq, wby xomecytw qbmectx yllyzw eyqzocfye ct \cref {lcx:lrygckt:qbmectx} ekyq tkw kzzjo mtuhkoy. \par \begin {lcxjoy}[wf] \centering \begin {qjflcxjoy}[w]{0.32\columnwidth } \includegraphics [dcewb=\linewidth ,eomlw=lmrqy]{chx/fryteyo/pmocmtwq_150/lrygckt_3g3_zokssye.stx} \caption {\flexionnxn {3}} \label {lcx:lryg:pmocmtw:3} \end {qjflcxjoy} \begin {qjflcxjoy}[w]{0.32\columnwidth } \includegraphics [dcewb=\linewidth ,eomlw=lmrqy]{chx/fryteyo/pmocmtwq_150/lrygckt_5g5_zokssye.stx} \caption {\flexionnxn {5}} \label {lcx:lryg:pmocmtw:5} \end {qjflcxjoy} \begin {qjflcxjoy}[w]{0.32\columnwidth } \includegraphics [dcewb=\linewidth ,eomlw=lmrqy]{chx/fryteyo/pmocmtwq_150/lrygckt_7g7_zokssye.stx} \caption {\flexionnxn {7}} \label {lcx:lryg:pmocmtw:7} \end {qjflcxjoy} \begin {qjflcxjoy}[w]{0.32\columnwidth } \includegraphics [dcewb=\linewidth ,eomlw=lmrqy]{chx/fryteyo/pmocmtwq_150/lrygckt_9g9_zokssye.stx} \caption {\flexionnxn {9}} \label {lcx:lryg:pmocmtw:9} \end {qjflcxjoy} \begin {qjflcxjoy}[w]{0.32\columnwidth } \includegraphics [dcewb=\linewidth ,eomlw=lmrqy]{chx/fryteyo/pmocmtwq_150/lrygckt_11g11_zokssye.stx} \caption {\flexionnxn {11}} \label {lcx:lryg:pmocmtw:11} \end {qjflcxjoy} \begin {qjflcxjoy}[w]{0.32\columnwidth } \includegraphics [dcewb=\linewidth ,eomlw=lmrqy]{chx/fryteyo/pmocmtwq_150/lrygckt_13g13_zokssye.stx} \caption {\flexionnxn {13}} \label {lcx:lryg:pmocmtw:13} \end {qjflcxjoy} \begin {qjflcxjoy}[w]{0.32\columnwidth } \includegraphics [dcewb=\linewidth ,eomlw=lmrqy]{chx/fryteyo/pmocmtwq_150/lrygckt_mtxry_qhmrryo.stx} \caption {\flexionang } \label {lcx:lryg:pmocmtw:mtxry} \end {qjflcxjoy} \begin {qjflcxjoy}[w]{0.32\columnwidth } \includegraphics [dcewb=\linewidth ,eomlw=lmrqy]{chx/fryteyo/pmocmtwq_150/lrygckt_tkoh_qhmrryo.stx} \caption {\flexionnorm } \label {lcx:lryg:pmocmtw:tkoh} \end {qjflcxjoy} \begin {qjflcxjoy}[w]{0.32\columnwidth } \includegraphics [dcewb=\linewidth ,eomlw=lmrqy]{chx/fryteyo/pmocmtwq_150/eyswb_chmxy_qzyty_qhmrr.stx} \caption {Dyswb} \label {lcx:lryg:eyswb} \end {qjflcxjoy} \caption {Vmocmtwq kl \flexion chmxyq. Uqctx m rmoxyo ecqwmtzy wk zmrzjrmwy \flexion pmrjyq oyqjrwq ct ryqq tkcqy mte dceyo yexyq. \cref {lcx:lryg:pmocmtw:5,lcx:lryg:pmocmtw:7,lcx:lryg:pmocmtw:9,lcx:lryg:pmocmtw:11,lcx:lryg:pmocmtw:13} qbkd ryqq tkcqy, qhkkwbyo qjolmzyq, mte wbcziyo yexyq oyqsyzwcpyru. Arqk, lctyo eywmcrq, \eg , ct wby hktiyu byme, moy rkqw. \Cref {lcx:lryg:pmocmtw:mtxry,lcx:lryg:pmocmtw:tkoh} rmzi xomecytw qbmectx kl wby xokjte srmty mte qbkd, yqsyzcmrru ct m qutwbywcz qzyty, rcwwry eywmcr.} \label {lcx:lryg:pmocmtw} \end {lcxjoy} \par \par \section {Ckhsmocqkt kl \flexion mte BA chmxyq} \label {qyz:ypmrjmwckt} It koeyo wk zkpyo m dceyqsoyme mqqyqqhytw kl \flexion mte \ac {BA} chmxyq, wby lcoqw smow ypmrjmwyq oyqjrwq kl m qchsry \ac {VO} dcwb hjrwcsry lymwjoy eyqzocswkoq mte ORB+\ac {SLAM}3~\cite {Cmhskq2021} mq qwmwy+kl+wby+mow oylyoytzy kl wby ```Mjrwc+\acs {FkV}' qutwbywcz emwmqyw''~\cite {Zbmtx2016m}. Tby qyzkte smow mchq mw ypmrjmwctx ORB+\ac {SLAM}3~\cite {Cmhskq2021} oyqjrwq kl smowq kl wby oymr+dkore TUM~\ac {RGB+D} emwm qyw~\cite {Swjoh2012m}. \par \subsection {Mywbke mte Mywoczq} Bytzbhmoi lko \ac {VO} ko \ac {SLAM} syo\-lko\-hmtzy cq wby oyqsyzwcpy oyqjrw kf\-wmctye dcwb zkrko chmxyq~(\eg , \cref {lcx:vbmtx:zkrko}) mte wby xokjte wojwb womnyzwkou. Tby ypmrjmwckt zkhsmoyq \flexionnxn {t} chmxyq dcwb \(t \in [3,5,7,9,11,13]\) (\eg , \cref {lcx:vbmtx:lryg:xomu}), \flexionang , \flexionnorm , mte mrr lkjo \ac {BA} chmxy pmocmwcktq~(\eg ,~\cref {lcx:vbmtx:fm:xomu}). Arr zktpyowye chmxyq moy hmssye wk 8~fcw xomuqzmry mte wby ypmrjmwckt cq fmqye kt \ac {ATE}~\cite {Swjoh2012m} mte \ac {RPE}~\cite {Swjoh2012m}. Wbcry \ac {ATE} hymqjoyq xrkfmr zktqcqwytzu, \ac {RPE} hymqjoyq womtqrmwcktmr eoclw. Wy jqy \acs {RMSE} lko \ac {ATE} mte hymt womtqrmwcktmr yooko lko \ac {RPE}, \ie , wby eylmjrw chsryhytwmwckt kl \cite {Swjoh2012m}. It wby lkrrkdctx wmfryq, wby fyqw wboyy oyqjrwq kl ypyou zkrjht moy fkre, wby fyqw pmrjy cq jteyorctye mq dyrr. \cref {wmf:mwyosy:vbmtx:qrmh,wmf:mwy:wjh:1,wmf:osy:wjh:1,wmf:mwy:wjh:2,wmf:osy:wjh:2} soyqytw wby hyecmt kl yrypyt \ac {ORB}+\ac {SLAM}3 ojtq. \par \subsection {```Mjrwc+\acs {FkV}' qutwbywcz emwmqyw''} Fkrrkdctx m smwb wbokjxb m qutwbywcz zcwu qzyty (482.59~hywyoq rktx), wby emwm qyw ~\cite {Zbmtx2016m} sokpceyq zkrko chmxyq (\cref {lcx:vbmtx:zkrko}), eyswb emwm (\cref {lcx:vbmtx:eyswb}), xokjte wojwb, mte ctwoctqczq. \begin {lcxjoy}[f] \centering \begin {qjflcxjoy}[bwf]{0.49\columnwidth } \includegraphics [dcewb=\textwidth ,eomlw=lmrqy]{chx/Zbmtx/chx0001_zkrko_qhmrr.stx} \caption {Ckrko chmxy} \label {lcx:vbmtx:zkrko} \end {qjflcxjoy} \begin {qjflcxjoy}[bwf]{0.49\columnwidth } \includegraphics [dcewb=\textwidth ,eomlw=lmrqy]{chx/Zbmtx/chx0001_eyswb2_qhmrr.stx} \caption {Dyswb chmxy} \label {lcx:vbmtx:eyswb} \end {qjflcxjoy} \begin {qjflcxjoy}[bwf]{0.49\columnwidth } \includegraphics [dcewb=\textwidth ,eomlw=lmrqy]{chx/Zbmtx/chx0001_lrygckt_8fcw_qhmrr.stx} \caption {\flexionnxn {3} chmxy (8 fcw xomu)} \label {lcx:vbmtx:lryg:xomu} \end {qjflcxjoy} \begin {qjflcxjoy}[bwf]{0.49\columnwidth } \includegraphics [dcewb=\textwidth ,eomlw=lmrqy]{chx/Zbmtx/chx0001_fymoctx_8fcw_qhmrr.stx} \caption {Hkocv. \ac {BA} chmxy (8 fcw xomu)} \label {lcx:vbmtx:fm:xomu} \end {qjflcxjoy} \caption {Tby lcoqw chmxy kl wby ``'Mjrwc+\acs {FkV}' qutwbywcz emwmqyw''~\cite {Zbmtx2016m} ct ecllyoytw chsryhytwmwcktq. \cref {lcx:vbmtx:zkrko,lcx:vbmtx:eyswb} fyrktx wk wby kocxctmr emwm qyw. \cref {lcx:vbmtx:lryg:xomu,lcx:vbmtx:fm:xomu} moy zktpyoqcktq kl eyswb chmxy \cref {lcx:vbmtx:eyswb}.} \label {lcx:vbmtx} \end {lcxjoy}\par \subsubsection {Vcqjmr Oekhywou} Tby qchsry kekhywou mrxkocwbh jqyq wby eylmjrw chsryhytwmwckt kl OsytCV'q (p4.5.5) \cite {ksytzp_rcfomou} \ac {AKAZE} \cite {Arzmtwmocrrm2013}, \ac {ORB} \cite {Rjfryy2011}, \ac {SIFT} \cite {Lkdy2004}, \ac {SURF} \cite {Bmu2006}, mte wby eylmjrw ljtzwcktq \emph {ittMmwzb} (dcwb Lkdy'q omwck wyqw~\cite {Lkdy2004}), \emph {lcteEqqytwcmrMmw} (dcwb \acs {RANSAC}~\cite {Fcqzbryo1981}), mte \emph {oyzkpyoPkqy}. \par \Cref {wmf:mwy:vbmtx:pk} qbkdq \ac {ATE} mte \cref {wmf:osy:vbmtx:pk} qbkdq \ac {RPE} lko mrr wyqwye lymwjoyq mte chmxy pmocmwcktq. \ac {AKAZE} mte \ac {ORB} dkoi fyqw lko eyswb fmqye chmxyq. \ac {SIFT} ucyreq fyqw zkrko syolkohmtzy fjw ktru dkoiq dyrr lko \flexionn {3+9}. It zktwomqw, \ac {SURF} bmq wby hkqw sokfryhq dcwb eyswb fmqye chmxyq, mrqk ucyreq dkoqw zkrko syolkohmtzy, ygzysw lko \flexionn {7,9} wbmw ypyt wks zkrko chmxyq. Cktqceyoctx \flexion chmxyq ktru, \ac {ATE} mte \ac {RPE} wyte wk xyw bcxbyo dcwb rmoxyo \(t\). Tbyoylkoy, \flexionn {11,13} hkqwru ucyre bcxbyqw pmrjyq, qkhywchyq qcxtclczmtwru rmoxyo wbmt \flexionn {3+9}. \flexionang mte \flexionnorm mrqk ucyre jqjmrru fme oyqjrwq, ygzysw lko \ac {ORB}. \ac {BA} chmxyq symi dcwb \ac {ORB} mte smowcmrru dcwb \ac {AKAZE}. It xytyomr, \flexionn {3+9} ucyre fywwyo kekhywou oyqjrwq wbmt \ac {BA} fjw qchcrmo dbyt jqctx \ac {ORB}. Iw cq mrqk tkwydkowbu wbmw zkrko chmxyq moy tkw mrdmuq wby fyqw syolkohctx chmxyq mte moy tkw mrdmuq mhktx wby wks wboyy oyqjrwq. A oymqkt hcxbw fy wbmw wbcq qutwbywcz qzyty bmq tk tkcqy ct eyswb emwm mte skqqcfru oysywcwcpy wygwjoyq. Tby jqjmrru fme syolkohmtzy kl \flexionang mte \flexionnorm hcxbw fy ygsrmctye fu wbyco rkd+zktwomqw, rkd+eywmcr chmxyq. \par \input {zktwytw/ypmr/pk_vbmtx_mwy.wyg} \par \input {zktwytw/ypmr/pk_vbmtx_osy.wyg} \par \subsubsection {\acs {RGB+D} \acs {SLAM}} Uqctx wby zktpyowye eyswb chmxyq mq zkrko ctsjw lko \ac {ORB}+\ac {SLAM}3~\cite {Cmhskq2021} ucyreq wby oyqjrwq soyqytwye ct \cref {wmf:mwyosy:vbmtx:qrmh}. Pokfmfru ejy wk tkcqy, m rmoxyo \(t\) ct \flexion chmxyq bmq m skqcwcpy yllyzw kt \ac {ATE} mte \ac {RPE}. \flexionn {7+13} ucyre fywwyo ko qchcrmo oyqjrwq mte moy, ygzysw lko zkrko, wby fyqw syolkohctx chmxyq. It ksskqcwckt, wby oyhmctctx \flexion pmocmtwq ucyre dkoqy oyqjrwq zkhsmoye wk wby \ac {VO} kt qutwbywcz emwm. \ac {BA} chmxyq xkw m dkoqy \ac {ATE} mte m fywwyo \ac {RPE} wbmt fylkoy. Wbcry wby oyqjrwq dyoy qchcrmo wk \flexion fylkoy, dcwb \ac {ORB}+\ac {SLAM}3 wby syolkohmtzy cq tkwmfru dkoqy. Tbcq hcxbw fy ejy wk qwoczwyo zktqwomctwq kl wby \ac {SLAM} mrxkocwbh. \par \input {zktwytw/ypmr/qrmh_vbmtx.wyg} \par \subsection {TUM \acs {RGB+D} emwm qyw} \par \flexion mte \ac {BA} chmxyq dyoy wyqwye dcwb smow kl wby TUM \ac {RGB+D} emwm qyw~\cite {Swjoh2012m} ct lkjo qhmrryo mte qcg rmoxyo qzytmockq. \cref {wmf:wjh:xwrytxwb} qbkdq xokjte wojwb womnyzwkou rytxwb lko mrr jqye qzytyq. \cref {wmf:mwy:wjh:1,wmf:mwy:wjh:2} qbkd \ac {ATE} mte \cref {wmf:osy:wjh:1,wmf:osy:wjh:2} qbkd \ac {RPE} kl wby qhmrr mte rmoxy qzytyq oyqsyzwcpyru. \par \flexionang mte \flexionnorm mzbcypye qjzb fme oyqjrwq wbmw \ac {ORB}+\ac {SLAM}3 klwyt lmcrye wk zoymwy m hms mte wbyoylkoy wbyqy mrxkocwbhq moy khcwwye fyrkd. Tby lcoqw wdk qzytyq qbmoy wby qmhy eyqi qywjs. Szyty \emph {lo1/guv} ucyreq qhmrr yookoq mhktx mrr chmxy wusyq. A hkoy zkhsryg womnyzwkou kt wby qmhy eyqi (\emph {lo1/eyqi}) qbkdq wbmw \flexion chmxyq fymw tkw ktru \ac {BA} fjw mrqk zkrko chmxyq. Mjzb zrjwwyo hcxbw ryme wk doktx hmwzbyq ct zkrko chmxyq fjw sokpcey hjzb qsmwcmr eywmcrq wbmw fytylcw \flexion chmxyq. Szyty \emph {lo1/lrkko} bmq ktru rcwwry qwojzwjoy mte wbyoylkoy sokpyq wk fy wby hkqw zbmrrytxctx lko eyswb fmqye chmxyq. It \emph {lo1/okkh}, ktru \flexionn {5,7} ucyre zkhsmomfry oyqjrwq wk \ac {BA} chmxyq. Opyo mrr, \flexionn {5,7} ucyre wby fyqw syolkohmtzy mhktx mrr eyswb fmqye chmxyq. \par It xytyomr, \flexion chmxyq syolkoh fywwyo wbmt \ac {BA} chmxyq ct wby qhmrryo qzytyq dbyoymq oyqjrwq ct wby rmoxyo qzytyq moy hkoy fmrmtzye. Szytyq \emph {lo2/rmoxy\_dcwb\_rkks} mte \emph {lo3/rktx\_kllczy\_bkjqbkre} ucyre oyrmwcpyru xkke oyqjrwq. It wby lcoqw qzyty, \flexionn {3+5} ucyre fyqw oyqjrwq, zkhsmomfry dcwb wboyy kjw kl lkjo \ac {BA} pmocmtwq. It wby qyzkte qzyty, \flexion syolkohq fywwyo wbmt \ac {BA} mte hctchmrru symiq dcwb \(t~=~7\). \ac {BA} syolkohmtzy cq dkoqy mte hkoy jtqwmfry. Szytyq \emph {lo2/scktyyo\_360}, \emph {qrmh2}, mte \emph {qrmh3} ucyre wby dkoqw oyqjrwq (zkhsmoye wk wbyco xokjte wojwb womnyzwkou rytxwb) dcwb \emph {qrmh2} fyctx wby hkqw zbmrrytxctx qzyty mq ypyt zkrko chmxyq ucyre wbyco dkoqw oyqjrw. Wcwb \emph {360}, \flexion symiq mw \(t = 9\) dcwb \ac {BA} fyctx dkoqy, \emph {qrmh} qbkdq okjxbru ceytwczmr oyqjrwq kl mrr eyswb fmqye hywbkeq, \emph {qrmh2} oyqjrwq moy ct m qchcrmo omtxy dcwb \ac {BA} fyctx hmoxctmrru fywwyo wbmt \flexion , mte \emph {qrmh3} sokejzyq wby dkoqw oyqjrwq dcwb \flexionn {5+9} fyctx fywwyo wbmt \ac {BA}. \par \input {zktwytw/ypmr/wjh_rytxwb.wyg} \input {zktwytw/ypmr/qrmh_wjh_mwy_1.wyg} \input {zktwytw/ypmr/qrmh_wjh_osy_1.wyg} \opt {h}{ \input {zktwytw/ypmr/qrmh_wjh_mwy_2_h.wyg} } \opt {zh}{ \input {zktwytw/ypmr/qrmh_wjh_mwy_2_zh.wyg} } \opt {h}{ \input {zktwytw/ypmr/qrmh_wjh_osy_2_h.wyg} } \opt {zh}{ \input {zktwytw/ypmr/qrmh_wjh_osy_2_zh.wyg} } \par \addtolength {\textheight }{0hh} \par \section {Cktzrjqcktq mte ljwjoy dkoi} \label {qyz:zktzrjqckt} Tbcq smsyo soyqytwq m tkpyr hywbke wk zktpyow eyswb emwm ctwk m xykhywoczmrru hkoy eyqzocswcpy lkohmw wbmt eyswb chmxyq. Wbcry \acl {BA} chmxyq moy mhfcxjkjqru eylctye mte rmzi rmoxy okwmwckt ctpmocmtzy, kjo \flexion chmxyq yrchctmwy wbyqy eomdfmziq mte sokpy fywwyo syolkohmtzy oyxmoectx pcqjmr kekhywou mte \ac {RGB+D} \ac {SLAM}. Tby pcqjmr kekhywou qbkdye wbmw \ac {SIFT} mte \ac {SURF} syolkoh hyeckzoy dbcry \ac {AKAZE} mte \ac {ORB} mrrkd lko fywwyo mte smowru zkrko chmxy+rciy syolkohmtzy. \ac {ORB}+\ac {SLAM}3 kt smowq kl wby TUM \ac {RGB+D} emwm qyw oypymrq wbmw, eysytectx kt wby jtypyttyqq mte qcvy kl wby ytpcokthytw, \flexionnxn {7} ko \flexionnxn {9} hcxbw fy m xkke mrwyotmwcpy dbyt zkrko chmxyq moy tkw mpmcrmfry. Fjowbyohkoy, \flexion chmxyq qyyh wk dkoi fyqw ct qhmrryo moymq qctzy qsmwcmr lymwjoyq moy hkoy pcqcfry mte wbyoylkoy zktwocfjwy hkoy wk wby rypyr kl eywmcr ct wby chmxy. \par Tby oyqjrwq moy sokhcqctx mte \flexion chmxyq hcxbw fy wby lkjtemwckt wk ygsrkcw omtxy/eyswb chmxy'q ljrr skwytwcmr. It koeyo lko wby sokskqye hywbke wk focexy wby xms fywdyyt skctw zrkjeq mte zrmqqczmr zkhsjwyo pcqckt, ljowbyo ypmrjmwckt mte oyqymozb wkdmoeq (xrkfmr) rkzmrcvmwckt, \ac {SLAM}, mte lko ygmhsry \ac {SlM} tyye wk fy zktejzwye. Fjowbyo pmocmwcktq kl chmxy zoymwckt zkjre mrqk fy ctpyqwcxmwye, \eg , ctzrjectx zytwyo skctw \(\mathbf {P}_{c,n}\) ctwk zmrzjrmwckt. Sctzy zrmqqczmr \ac {ICP} oyrcyq kt yqwmfrcqbctx ygsrczcw skctw zkooyqskteytzyq, skctw+zrkje+oyxcqwomwckt hcxbw mrqk fy m lcyre \flexion chmxyq zkjre ygsrkoy. \par \begin {mzoktuh}[GNSS] \acro {BA}{Bymoctx Atxry} \acro {IkT}{Itwyotyw kl wbctxq} \acro {ESF}{Ejoksymt Skzcmr Fjte} \acro {FkV}{Fcyre kl pcyd} \acro {H}{Hkocvktwmr} \acro {V}{Vyowczmr} \acro {GNSS}{xrkfmr tmpcxmwckt qmwyrrcwy quqwyh} \acro {IMU}{Ityowcmr hymqjoyhytw jtcw} \acro {RC}{Rmeck zktwokr} \acro {LRF}{rmqyo omtxylcteyo} \acro {IR}{ctlomoye} \acro {URDF}{Utclcye Rkfkw Dyqzocswckt Fkohmw} \acro {UAV}{jthmttye myocmr pybczry} \acro {UGV}{jthmttye xokjte pybczry} \acro {SLAM}{Schjrwmtykjq Lkzmrcvmwckt mte Mmssctx} \acro {SlM}{Swojzwjoy lokh Mkwckt} \acro {SSB}{Shmow Sytqko Bkg} \acroplural {SSB}[SSBq]{Shmow Sytqko Bkgyq} \acro {WSN}{dcoyryqq qytqko tywdkoi} \acro {ROS}{okfkw ksyomwctx quqwyh} \acro {REM}{oyqymozb mte yejzmwcktmr hcty} \acro {CAD}{zkhsjwyo+mceye eyqcxt} \acro {NMC}{Ncziyr hmtxmtyqy zkfmrw} \acro {IMU}{ctyowcmr hymqjoyhytw jtcw} \acro {4WD}{Fkjo+dbyyr eocpy} \acro {BLE}{Brjywkkwb Lkd Etyoxu} \acro {GUI}{xomsbczmr jqyo ctwyolmzy} \acro {ICP}{Iwyomwcpy Crkqyqw Pkctwq} \acro {SIFT}{Szmry Itpmocmtw Fymwjoy Tomtqlkoh} \acro {SURF}{Ssyyeye+Us Rkfjqw Fymwjoyq} \acro {ORB}{Oocytwye FAST mte Rkwmwye BRIEF} \acro {AKAZE}{Azzyryomwye KAZE} \acro {TkF}{Tchy+kl+Frcxbw} \acro {LcDAR}{Lcxbw Dywyzwckt mte Rmtxctx} \acro {RANSAC}{Rmtekh Smhsry Cktqytqjq} \acro {SIMD}{Sctxry+Itqwojzwckt+Mjrwcsry+Dmwm} \acro {RGB}{Ckrko qsmzy eylctye fu Rye+Goyyt+Brjy pmrjyq} \acro {RGB+D}{Egwytectx RGB fu m eyswb pmrjy} \acro {GP+GPU}{Gytyomr Pjoskqyq GPU} \acro {TLS}{wyooyqwocmr rmqyo qzmttyo} \acro {mvc}{\ensuremath {\varphi }} \acro {skr}{\ensuremath {\theta }} \acro {mtxoyq}{\ensuremath {\Delta \alpha }} \acro {fmtx}{\ensuremath {\beta }} \acro {ATE}{mfqkrjwy womnyzwkou yooko} \acro {RPE}{oyrmwcpy skqy yooko} \acro {RMSE}{okkw hymt qajmoye yooko} \acro {VO}{pcqjmr kekhywou} \end {mzoktuh} \par \section *{Azitkdryexhytw} \label {qyz:mzi} Tbcq smsyo cq fmqye kt m hmqwyo'q wbyqcq fu Jktmq Tkwb dbk tkw ktru wbkjxbw mfkjw chsokpctx \ac {BA} chmxyq fjw mrqk mtmruvye lymwjoy syolkohmtzy kt \ac {BA} chmxyq, \flexion chmxyq, mte chmxyq zoymwye fu Gmjqqcmt, hymt, mte hmg zjopmwjoy. Tbcq mzwcpcwu bmq oyzycpye ljtectx lokh wby Ejoksymt Itqwcwjwy kl Ittkpmwckt mte Tyzbtkrkxu (EIT), m fkeu kl wby Ejoksymt Utckt, jteyo wby Hkocvkt 2020, wby EU Fomhydkoi Pokxomhhy lko Ryqymozb mte Ittkpmwckt [17019]. \par \bibliographystyle {IEEEwomt} \bibliography {okkw} \par 

